From Prompts to Templates: A Systematic Prompt Template Analysis for Real-world LLMapps

Large Language Models (LLMs) have revolutionized human-AI interaction by enabling intuitive task execution through natural language prompts. Despite their potential, designing effective prompts remains a significant challenge, as small variations in structure or wording can result in substantial differences in output. To address these challenges, LLM-powered applications (LLMapps) rely on prompt templates to simplify interactions, enhance usability, and support specialized tasks such as document analysis, creative content generation, and code synthesis. However, current practices heavily depend on individual expertise and iterative trial-and-error processes, underscoring the need for systematic methods to optimize prompt template design in LLMapps. This paper presents a comprehensive analysis of prompt templates in practical LLMapps. We construct a dataset of real-world templates from open-source LLMapps, including those from leading companies like Uber and Microsoft. Through a combination of LLM-driven analysis and human review, we categorize template components and placeholders, analyze their distributions, and identify frequent co-occurrence patterns. Additionally, we evaluate the impact of identified patterns on LLMs' instruction-following performance through sample testing. Our findings provide practical insights on prompt template design for developers, supporting the broader adoption and optimization of LLMapps in industrial settings.

==> figures/excluded_prompts.tex <==
\chapter{Representative Prompts Guidelines}\label{chapter:representative}
Table \ref{tab:prompts_excluded} shows some examples of prompts excluded from our analysis. Prompts that are too short or contain only an external path are automatically filtered out, while the other two types are manually removed.
\begin{longtable}{p{3cm} p{13cm}}
\caption[Examples of prompts excluded from our analysis]{Examples of prompts excluded from our analysis.}\label{tab:prompts_excluded}\\
\toprule
\textbf{Category} & \textbf{Prompts not included in our anaysis}\\
\midrule
\multirow{5}{=}{Too Short} & - "instructions" \\
&-"\textbackslash n None Input Action \textbackslash n" \\
& - "<<<<CLAIM>>>>" \\
& - "[('system', PLACEHOLDER), ('human', PLACEHOLDER)]" \\
                              & ...\\
\midrule
\multirow{5}{=}{External URL/File/Documentation Path} & - "joplin://x-callback-url/openNote?id={id}" \\
                              & - "meeting\_summarizer/prompts/summarize\_transcript.txt"\\
                              & - "/home/adithya/sem6/review-sum/prompts"\\
                              & -"sematic/examples/hackernews\_summarization/template.html"\\
                              & ...\\
\midrule
\multirow{3}{=}{False Positives}  
                                       & - description of the class is regonized as prompts(e.g., prompts from the repository named "ai-forever/gigachain","homanp/superagent")\\        
                                       & ...\\
\midrule

\multirow{5}{=}{Contains Other Languages} &  \\
                                         & - \begin{CJK*}{UTF8}{gbsn}"一口井7米深，有只蜗牛从井底往上爬，白天爬3米，晚上往下坠2米。问蜗牛几天能从井里爬出来？Let's work this out in a step by step way to be sure we have the right answer."\end{CJK*} \\
                                         & ... \\
\bottomrule
\end{longtable}

==> sections/Analysis.tex <==
\section{Analysis}
\subsection{Research Questions}
In this section, we address the following research questions:
\begin{itemize}
    \item \textbf{RQ1: What are the common task themes and constituent components in prompt templates?}
    
    We classify themes and analyze components within the collected prompt templates, identifying typical ordering patterns across various prompt components.
    \item \textbf{RQ2: What specific words and phrases are frequently used in different components, and are there common construction patterns?}
    
    We examine word- and phrase-level content within components, identifying patterns that play critical roles in shaping both response format and content.
    \item \textbf{RQ3: How do placeholders vary in terms of types and positions within prompt templates?}
    
    We categorize placeholders and investigate their relative positions, examining positional patterns both among placeholders and in relation to prompt components.
    \item \textbf{RQ4: How do different construction patterns in prompt templates influence LLMs' instruction-following abilities?}
    
    We sample prompt templates with specific patterns, populate them with sample data, and generate outputs to assess the effectiveness of these patterns on LLMs' instruction-following ability through human evaluation.
\end{itemize}

\subsection{RQ1: Identifying Themes and Components in Prompt Templates}
\begin{figure}[htpb]
    \centering
    \scriptsize 
    \renewcommand{\arraystretch}{0.55}
    \subfloat[][Pattern A.]{ 
        \begin{tabular}{|@{\hskip 5pt}p{0.81\linewidth}@{\hskip 5pt}|p{0.14\linewidth}@{}}
            \cline{1-1}
            \\
            \textcolor{TUMBlue}{You are an AI assistant acting as a content advisor for a tech blog.}  
            \textcolor{TUMAccentGreen}{Suggest two relevant blog topics based on recent trends in \textbf{\{subject\_area\}}.} 
            & \textcolor{TUMBlue}{\textbf{Profile/Role}} \textcolor{TUMAccentGreen}{\textbf{Directive}}  \\
            \\
            \textcolor{TUMAccentOrange}{You are given the following information:} & \textcolor{TUMAccentOrange}{\textbf{Context}} \\
            \textcolor{TUMAccentOrange}{- The blog focuses on topics related to \textbf{\{subject\_area\}.}} &  \\
            \textcolor{TUMAccentOrange}{- Recent posts on \textbf{\{high\_engagement\_topics\}} have received high engagement.} &  \\
            \\
            \begin{minipage}[t]{\linewidth}
            \textcolor{TUMAccentBlue}{To complete this task, follow these steps:}\\
                \textcolor{TUMAccentBlue}{1. Review the provided context and analyze current trends in \textbf{\{subject\_area\}}.} \\
                \textcolor{TUMAccentBlue}{2. Suggest two blog topics that align with the blog’s focus and audience.} \\
                \textcolor{TUMAccentBlue}{3. Ensure the suggested topics are relevant to the recent engagement trends, particularly \textbf{\{high\_engagement\_topics\}}, and are accessible to a general audience.}
            \end{minipage} & \textcolor{TUMAccentBlue}{\textbf{Workflows}} \\
            \\
            \textcolor{TUMDarkGray}{Avoid overly technical or niche topics that may overwhelm readers. Keep topics broad and engaging for non-experts.} & \textcolor{TUMDarkGray}{\textbf{Constraints}} \\
            \\
            \begin{minipage}[t]{\linewidth}
                \textcolor{TUMGray}{Provide your response in the following format:} \\
                \textcolor{TUMGray}{Topic 1: [Title] - [One-sentence explanation]} \\
                \textcolor{TUMGray}{Topic 2: [Title] - [One-sentence explanation]}
            \end{minipage} & \textcolor{TUMGray}{\textbf{Output Format/Style}} \\
            \\
            \begin{minipage}[t]{\linewidth}
            \textcolor{TUMSecondaryBlue}{There are two example topics based on trends in AI:} \\
                \textcolor{TUMSecondaryBlue}{Topic 1: AI in Public Services - Discuss how AI is being used to enhance efficiency in public services like healthcare and education.} \\
                \textcolor{TUMSecondaryBlue}{Topic 2: Ethical AI in Automation - Explore the ethical implications of AI-driven automation in industries like manufacturing and logistics.}
            \end{minipage} &  \textcolor{TUMSecondaryBlue}{\textbf{Examples}} \\
            \\
            \cline{1-1}
        \end{tabular}
        \label{fig:pattern_a}
    }
    \quad 
    \subfloat[][Pattern B.]{
        \begin{tabular}{|p{\linewidth}|}
            \cline{1-1}
            \\
            \textcolor{TUMBlue}{You are an AI system designed to generate data analysis reports.}  
            \textcolor{TUMAccentGreen}{Generate a detailed report based on the analysis of \textbf{\{data\_type\}} from \textbf{\{time\_range\}}.} 
           \\
            \\
            \begin{minipage}[t]{\linewidth}
                \textcolor{TUMGray}{Provide the report in the following structured format:} \\
                \textcolor{TUMGray}{\{ "summary": "Brief summary of key findings", "insights": [ "Insight 1", "Insight 2", "Insight 3" ], "recommendations": [ "Recommendation 1", "Recommendation 2" ] \}} \\
            \end{minipage}  \\
            
            \textcolor{TUMDarkGray}{Ensure the report includes diverse insights from different aspects of the data. The analysis should provide a balance between high-level trends and deep-dive insights into anomalies or outliers.}  \\
            \\
            \textcolor{TUMAccentOrange}{The dataset covers a period of \{time\_range\} and includes key metrics related to \{data\_type\}. The report should highlight any significant patterns or anomalies.} \\
            \\
            \begin{minipage}[t]{\linewidth}
            \textcolor{TUMAccentBlue}{Follow these steps:}\\
                \textcolor{TUMAccentBlue}{1. Analyze the dataset to identify major trends and outliers.} \\
                \textcolor{TUMAccentBlue}{2. Summarize the key findings and generate actionable insights based on the analysis.}
            \end{minipage}  \\
            \\
          \begin{minipage}[t]{\linewidth}
        \textcolor{TUMSecondaryBlue}{Example output:} \\
        \textcolor{TUMSecondaryBlue}{\{"summary": "The dataset shows consistent growth in the first half of the year, with a notable anomaly in Q2.",\\
        "insights": [ 
            "Insight 1: Overall performance improved by 15\% compared to the same period last year.", 
            "Insight 2: There was a significant dip in performance during May due to external factors, particularly in the retail sector.", 
            "Insight 3: Despite the dip in May, Q3 showed signs of recovery, with key metrics returning to baseline." ],\\
        "recommendations": [ 
            "Recommendation 1: Further investigate the cause of the May anomaly and explore strategies to mitigate future risks.", 
            "Recommendation 2: Focus on maintaining steady growth through Q4 by diversifying market strategies." ] \}} \\
    \end{minipage}
     \\
            \cline{1-1}
        \end{tabular}
        \label{fig:pattern_b}
    }
    \caption{Examples of two different patterns.}
    \label{fig:pattern_all_elements}
\end{figure}

In RQ1, we first investigate into the theme distribution and component composition of the representative prompts extracted from LLM-powered applications. Based on these findings, we further analyze the component co-occurrence patterns.

\noindent \textbf{Theme of Prompts.} 
\begin{figure}[htpb]
    \centering
      \includegraphics[width=\linewidth]{figures/theme_method_3.png}
    \caption{Relative frequency distribution of prompt themes.}
    \label{fig:theme_classification_3}
\end{figure}
Figure~\ref{fig:theme_classification_3} shows the theme distribution of the collected prompts. Among the twelve theme categories, "Information Seeking" accounts for 42.2\%, significantly more than any other category. The second most common category is "Editing", with 11.6\%, indicating that developers often leverage the model's analytical processing capabilities to refine and improve the existing text. This suggests that using the model in scenarios involving given text is particularly popular, as it helps minimize the risk of generating hallucinations by basing the output on verified information provided by developers or end-users. Additionally, information seeking tasks are well-suited for Retrieval-Augmented Generation (RAG), which combines retrieval from external knowledge bases with generation, ensuring that the model provides accurate and relevant responses based on verified data.

Meanwhile, "Coding \& Debugging" is the third most common category, accounting for 10.3\%. This popularity can be attributed to the model's proven effectiveness in understanding and working with code, as demonstrated by successful applications (\eg, Copilot\cite{github_copilot}, Cursor\cite{cursor_ai}). These tools showcase the model's capacity to handle code-related tasks efficiently, making this a prevalent application area for LLMs.


% \begin{figure}
%     \centering
% \includegraphics[width=0.5\textwidth]{figures/theme_classification_result_method_3.png}
%     \caption{\junjie{Theme classification result. (v1)}}
%     \label{fig:theme_classification}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/theme.png}
%     \caption{\junjie{Theme classification result.(v2)}}
%     \label{fig:theme_classification_2}
% \end{figure}

\noindent \textbf{Distribution and Positional Patterns of Components. }
Figure \ref{fig:element_distribution} shows the detection results for the seven categories of components, indicating how frequently each appears in all prompts. Among these components, the four most common are Directive, Context, Output Format/Style, and Constraints. The Directive represents the task intent of the prompt, guiding the language model on how to perform a task. Most prompts require a clear and complete directive to instruct the model effectively. The Context typically includes the input content and relevant contextual descriptions, helping the model understand the task in detail. Given that these prompt templates are designed for LLM-based applications, developers often specify an Output Format/Style (\eg, Json format) and set Constraints (\eg, length, number of result). This ensures the generated content is more predictable, easier for downstream applications to process, and maintains consistency across outputs.

\begin{figure}[htpb]
    \centering
      \includegraphics[width=\linewidth]{figures/element/element_distribution.png} 
    \caption{Relative frequency distribution of different prompt components.}
    \label{fig:element_distribution}
\end{figure}
\begin{figure}[htpb]
    \centering
     \includegraphics[width=\linewidth]{figures/sequence/element_transition.png} 
    \caption{Component transition probability matrix.}
    \label{fig:element_transition}
\end{figure}


\begin{comment}
\begin{figure}[htpb]
    \centering
    \subfloat[][\junjie{Frequency of different elements.}\mao{\sout{Better to put them up and down, and make the grid figure larger}}]{
    \includegraphics[width=0.7\textwidth]{figures/element/element_distribution.png} \label{fig:element_distribution}}
    \quad\quad\quad
    \subfloat[][\junjie{Element transition probability matrix.}\mao{\sout{Use one figure of 2 real case with labeled elements to illustrate these two patterns. If no such prompt in dataset, we can just let LLM to construct cases for illustration.}}]{
    \includegraphics[width=0.7\textwidth]{figures/sequence/element_transition.png}    \label{fig:element_transition}}
    \caption[]{}
    \label{fig:element}
\end{figure}
\end{comment}

We also investigate the relative positions of various components. As shown in Figure \ref{fig:element_transition}, both the X and Y axes represent the different component types, with each coordinate point indicating the probability that component X follows component Y. The darker the color, the higher the probability that this positional pattern occurs. For example, Context is most likely to be followed by Directive with a probability of 0.48. Based on these results, we identify two common component combination patterns (assuming that each component appears exactly once), and Figure~\ref{fig:pattern_all_elements} providing specific prompt examples for each pattern: 
 \begin{itemize}
    \item \textbf{Pattern A:} Profile/Role -> Directive -> Context -> Workflows -> Constraints -> Output Format/Style -> Examples.
     \item \textbf{Pattern B:} Profile/Role -> Directive -> Output Format/Style -> Constraints -> Context -> Workflows -> Examples.
\end{itemize}

% \begin{figure}[htpb]
%     \centering
%     \scriptsize 
%     \renewcommand{\arraystretch}{0.8}
%     \begin{tabular}{|@{\hskip 5pt}p{0.77\textwidth}@{\hskip 5pt}|p{0.18\textwidth}@{}}
%         \cline{1-1}
%         \\
%         \textcolor{TUMAccentOrange}{Here is a text description of a behavior:} \newline
%         \textcolor{TUMAccentOrange}{\textit{PLACEHOLDER}} \\
%         \textcolor{TUMAccentOrange}{And here is the description of some entities from the \textit{PLACEHOLDER}:} \newline
%          \textcolor{TUMAccentOrange}{\textit{PLACEHOLDER}} & \textcolor{TUMAccentOrange}{\textbf{Context}} \\
%         \\
%         \textcolor{TUMAccentGreen}{From those entities, return a reranked list with the 10 most relevant entities to the text description ordered from most relevant to least relevant.} & \textcolor{TUMAccentGreen}{\textbf{Directive}} \\
%         \\
%         \textcolor{TUMDarkGray}{If an component does not seem related enough, do not include it in the list.} & \textcolor{TUMDarkGray}{\textbf{Constraints}} \\
%         \\
%         \textcolor{TUMGray}{The format of the output list should be in JSON style and include only the ids of the entities in the list, not the names or definitions.} & \textcolor{TUMGray}{\textbf{Output Format/Style}} \\
%         \\
%         \cline{1-1}
%     \end{tabular}
%     \caption{\junjie{An example illustrating the use of the four most common components for an Information Retrieval task.}}
%     \label{fig:specific_example}
% \end{figure}

\begin{tcolorbox}[colback=black!5!white,colframe=black!75!black,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm},left=0.1pt, right=0.1pt]
\textbf{Answer to RQ1:} Our analysis identifies Information Seeking, Editing, and Code \& Debugging as the three most common themes in prompt templates, each constituting over 10\% of the dataset. Similarly, Directive, Context, Output Format/Style, and Constraints are the most frequently utilized prompt components, each also exceeding 10\%. Through the examination of co-occurrence and positional patterns, we discover two general arrangement patterns for organizing prompt components, applicable across all component types.
\end{tcolorbox}

% Additionally, we observe that the probabilities for directive followed by context and context followed by directive are the highest among all element sequences. To explore this further, we conduct a sequence analysis of prompts containing two elements. The results indicate different positional patterns for directive, context. Figure~\ref{fig:directive_context} shows the percentage occurrence of these two patterns in both the overall dataset and in prompt templates of "Coding \& Debugging" theme. In the overall dataset, the occurrence probabilities of these two patterns are similar, with directive followed by context being slightly more common. However, in the "Coding \& Debugging" theme prompt templates, the probability of context followed by directive is significantly higher compared to the opposite order.

% \begin{figure}[htpb]
%     \centering
%     \subfloat[][Overall.]{
%     \includegraphics[width=0.45\textwidth]{figures/sequence/directive_context_overall.png} \label{fig:directive_context_overall}}
%     \quad
%     \subfloat[][Coding \& Debugging.]{
%     \includegraphics[width=0.45\textwidth]{figures/sequence/directive_context_coding.png}    \label{fig:directive_context_coding}}
%     \caption[]{Different positional pattern for directive -> context and context -> directive.}
%     \label{fig:directive_context}
% \end{figure}

% We believe this difference is due to the nature of coding tasks. Figure~\ref{fig:prompt_templates_coding} illustrates two examples of prompt templates from the "Coding \& Debugging" theme. In these cases, the context often consists of code, which is a highly structured form of text involving variables, function names, and data structures. Presenting the code first allows the model to understand the structural information before being given the specific directive on how to proceed. This approach makes it easier for the model to apply structural knowledge effectively to complete the task at hand. 

% \begin{figure}[htpb]
%     \centering
%     \subfloat[][Prompt template for fixing a JavaScript issue.]{ 
%         \fbox{
%         \parbox{0.44\textwidth}{
%         Given a JavaScript code issue with the following description: \newline
%         \textbf{\{issue\_description\}} \newline
%         Provide a code change to fix this issue:
%         }
%         }
%     }
%     \quad 
%     \subfloat[][Prompt template for summarizing code arguments and variables.]{ 
%         \fbox{
%         \parbox{0.44\textwidth}{
%         Here is the part of the code that you are supposed to continue: \newline
%         \textbf{\{code\_snippets\}} \newline
%         Write a summarize function for the argument name and variable below: \newline
%         Argument Name: \textbf{\{argument\}} \newline
%         Variable Name: \textbf{\{variable\}} \newline
%         Summarization Code:
%         }
%         }
%     }
%     \caption{Examples of prompt templates of "Coding \& Debugging" theme, where the context is provided first, followed by a directive. }
%     \label{fig:prompt_templates_coding}
% \end{figure}

\begin{comment}
\begin{figure}
    \centering
\includegraphics[width=0.7\textwidth]{figures/element_co_occurance.png}
    \caption{\junjie{Network graph of element co-occurrence. (directive is the most frequently used, followed by context. Strong dependency between directive and context, directive and output format.)}\mao{\sout{Is it the result for element detection in 4167 prompts? The number of directive seems not that many.}}}
    \label{fig:element_co_occurance}
\end{figure}
\end{comment}




\begin{comment}
    \begin{figure}
    \centering
\includegraphics[width=0.7\textwidth]{figures/sequence/element_transition.png}
    \caption{\junjie{Element transition probability matrix. (1. profile-> directive->context->workflow->constraints->output format/style->example
2. profile-> directive-> output format->constraints->context->workflow->example
)}\mao{Use one figure of 2 real case with labeled elements to illustrate these two patterns. If no such prompt in dataset, we can just let LLM to construct cases for illustration.}\junjie{no real case}}
    \label{fig:element_transition}
\end{figure}
\end{comment}
\begin{comment}
\begin{figure}[!h]
    \centering
    \begin{tabular}{|@{\hskip 10pt}p{0.75\textwidth}@{\hskip 10pt}|p{0.15\textwidth}@{}}
        \cline{1-1}
        \\
        \textcolor{TUMBlue}{You are an AI assistant acting as a content advisor for a tech blog.}  \textcolor{TUMAccentGreen}{Suggest two relevant blog topics based on recent trends in \textbf{\{subject\_area\}}.} & \textcolor{TUMBlue}{\textbf{Profile/Role}} \textcolor{TUMAccentGreen}{\textbf{Directive}}  \\
        \\
        \textcolor{TUMAccentOrange}{You are given the following information:} & \textcolor{TUMAccentOrange}{\textbf{Context}} \\
        \textcolor{TUMAccentOrange}{- The blog focuses on topics related to \textbf{\{subject\_area\}.}} &  \\
         \textcolor{TUMAccentOrange}{- Recent posts on \textbf{\{high\_engagement\_topics\}} have received high engagement.} &  \\
         \\
        \begin{minipage}[t]{\linewidth}
         \textcolor{TUMAccentBlue}{To complete this task, follow these steps:}\\
            \textcolor{TUMAccentBlue}{1. Review the provided context and analyze current trends in \textbf{\{subject\_area\}}.} \\
            \textcolor{TUMAccentBlue}{2. Suggest two blog topics that align with the blog’s focus and audience.} \\
            \textcolor{TUMAccentBlue}{3. Ensure the suggested topics are relevant to the recent engagement trends, particularly \textbf{\{high\_engagement\_topics\}}, and are accessible to a general audience.}
        \end{minipage} & \textcolor{TUMAccentBlue}{\textbf{Workflows}} \\
        \\
        \textcolor{TUMDarkGray}{Avoid overly technical or niche topics that may overwhelm readers. Keep topics broad and engaging for non-experts.} & \textcolor{TUMDarkGray}{\textbf{Constraints}} \\
        \\
        \begin{minipage}[t]{\linewidth}
            \textcolor{TUMGray}{Provide your response in the following format:} \\
            \textcolor{TUMGray}{Topic 1: [Title] - [One-sentence explanation]} \\
            \textcolor{TUMGray}{Topic 2: [Title] - [One-sentence explanation]}
        \end{minipage} & \textcolor{TUMGray}{\textbf{Output Format/Style}} \\
        \\
        \begin{minipage}[t]{\linewidth}
        \textcolor{TUMSecondaryBlue}{There are two example topics based on trends in AI:} \\
            \textcolor{TUMSecondaryBlue}{Topic 1: AI in Public Services - Discuss how AI is being used to enhance efficiency in public services like healthcare and education.} \\
            \textcolor{TUMSecondaryBlue}{Topic 2: Ethical AI in Automation - Explore the ethical implications of AI-driven automation in industries like manufacturing and logistics.}
        \end{minipage} &  \textcolor{TUMSecondaryBlue}{\textbf{Examples}} \\
        \\
        \cline{1-1}
    \end{tabular}
    \caption{\junjie{Example of profile/role -> directive ->context ->workflows ->constraints ->output format/style->examples.}\mao{Better to make the example shorter and make the figure smaller, two examples less than one page will be suitable.}}
     \label{fig:example_all_elements_1}
\end{figure}

\begin{figure}[!h]
    \centering
    \begin{tabular}{|@{\hskip 10pt}p{0.75\textwidth}@{\hskip 10pt}|p{0.15\textwidth}@{}}
        \cline{1-1}
        \\
        \textcolor{TUMBlue}{You are an AI system designed to generate data analysis reports.}  
        \textcolor{TUMAccentGreen}{Generate a detailed report based on the analysis of \textbf{\{data\_type\}} from \textbf{\{time\_range\}}.} 
        & \textcolor{TUMBlue}{\textbf{Profile/Role}} \textcolor{TUMAccentGreen}{\textbf{Directive}} \\
        \\
        \begin{minipage}[t]{\linewidth}
            \textcolor{TUMGray}{Provide the report in the following structured format:} \\
            \textcolor{TUMGray}{\{ "summary": "Brief summary of key findings", "insights": [ "Insight 1", "Insight 2", "Insight 3" ], "recommendations": [ "Recommendation 1", "Recommendation 2" ] \}} \\
        \end{minipage} & \textcolor{TUMGray}{\textbf{Output Format/Style}} \\
        \\
        \textcolor{TUMDarkGray}{Ensure the report includes diverse insights from different aspects of the data. The analysis should provide a balance between high-level trends and deep-dive insights into anomalies or outliers.} & \textcolor{TUMDarkGray}{\textbf{Constraints}} \\
        \\
        \textcolor{TUMAccentOrange}{The dataset covers a period of \{time\_range\} and includes key metrics related to \{data\_type\}. The report should highlight any significant patterns or anomalies.} & \textcolor{TUMAccentOrange}{\textbf{Context}} \\
        \\
        \begin{minipage}[t]{\linewidth}
         \textcolor{TUMAccentBlue}{Follow these steps:}\\
            \textcolor{TUMAccentBlue}{1. Analyze the dataset to identify major trends and outliers.} \\
            \textcolor{TUMAccentBlue}{2. Summarize the key findings and generate actionable insights based on the analysis.}
        \end{minipage} & \textcolor{TUMAccentBlue}{\textbf{Workflows}} \\
        \\
      \begin{minipage}[t]{\linewidth}
    \textcolor{TUMSecondaryBlue}{Example output:} \\
    \textcolor{TUMSecondaryBlue}{\{"summary": "The dataset shows consistent growth in the first half of the year, with a notable anomaly in Q2.",\\
    "insights": [ 
        "Insight 1: Overall performance improved by 15\% compared to the same period last year.", 
        "Insight 2: There was a significant dip in performance during May due to external factors, particularly in the retail sector.", 
        "Insight 3: Despite the dip in May, Q3 showed signs of recovery, with key metrics returning to baseline." ],\\
    "recommendations": [ 
        "Recommendation 1: Further investigate the cause of the May anomaly and explore strategies to mitigate future risks.", 
        "Recommendation 2: Focus on maintaining steady growth through Q4 by diversifying market strategies." ] \}} \\
\end{minipage}
 &  \textcolor{TUMSecondaryBlue}{\textbf{Examples}} \\
        \\
        \cline{1-1}
    \end{tabular}
    \caption{\junjie{Example of profile/role -> directive -> output format -> constraints -> context -> workflows -> examples.}}
     \label{fig:example_all_elements_2}
\end{figure}
\end{comment}
\begin{comment}
    \begin{figure}[htpb]
    \centering
    \subfloat[][3 elements.]{
    \includegraphics[width=0.8\textwidth]{figures/sequence/3_elements.png} \label{fig:sequence_3}}
    \quad\quad\quad
    \subfloat[][4 elements.]{
    \includegraphics[width=0.8\textwidth]{figures/sequence/4_elements.png}    \label{fig:sequence_4}}
    \caption[]{\junjie{Frequency of elements in each position overall (first occurrence only). Common starting elements:
In prompts with 3 and 4 elements, the Profile/role and Directive elements usually appear in the first position.
Common ending elements: Output format/style and Constraints often appear in the last position.
Mid-Sequence elements: Context and workflow are frequently found in the middle of the sequences.
}}
    \label{fig:element_position_overall}
\end{figure}
\end{comment}


\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/directive/directive_type.png}
    \caption{Directive type distribution. \junjie{("prompts can be either question-style or instruction-style" ref1: https://arxiv.org/pdf/2305.11430 ref2: https://arxiv.org/pdf/2406.06608)}}
    \label{fig:directive_type}
\end{figure}    

\begin{figure}[htpb]
    \centering
    \subfloat[][Information seeking.]{
    \includegraphics[width=0.45\textwidth]{figures/directive/directive_information_seeking.png}\label{fig:directive_info}}
    \quad\quad\quad
    \subfloat[][Creative writing.]{\includegraphics[width=0.45\textwidth]{figures/directive/directive_creative_writing.png}\label{fig:directive_writing}}
    \quad\quad\quad
    \subfloat[][Editing.]{\includegraphics[width=0.45\textwidth]{figures/directive/directive_editing.png}\label{fig:directive_editing}}
    \quad\quad\quad
    \subfloat[][Reasoning.]{\includegraphics[width=0.45\textwidth]{figures/directive/directive_reasoning.png}\label{fig:directive_reasoning}}
    \quad\quad\quad
    \subfloat[][Coding \& Debugging.]{\includegraphics[width=0.45\textwidth]{figures/directive/directive_coding_debugging.png}\label{fig:directive_coding}}
    \quad\quad\quad
    \subfloat[][Data analysis.]{\includegraphics[width=0.45\textwidth]{figures/directive/directive_data_analysis.png}\label{fig:directive_data}}
    \caption[]{\junjie{Most common root verbs and their top direct noun objects.}}
    \label{fig:directive_verb_noun}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/profile_role_phrases.png}
    \caption{\junjie{Distribution of description sentences(>=5 words) of profile/role. Direct role definitions such as "you are an..." and "you are a..." are the most common patterns; Task-oriented descriptions: "your task is to...", "your job is to...",  "you are going to.."; Command-like descriptions (instruct or remind the role about its duties or behavior): "I want you to act..." and ”never forget you are a..." ; Contextual Role Description: "as a …"}}
    \label{fig:profile_role_description}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figures/output_format/output_format_style_distribution.png}
    \caption{\junjie{Distribution of output format/style.}}
    \label{fig:output_distribution}
\end{figure}   
\end{comment}


% \begin{figure}[htpb]
%     \centering
%     \subfloat[][Word cloud.]{
%     \includegraphics[width=0.4\textwidth]{figures/output_format/word_cloud_output_format_overall.png} \label{fig:output_word}}
%     \quad\quad\quad
%     \subfloat[][Distribution by category.]{
%     \includegraphics[width=0.4\textwidth]{figures/output_format/top_output_format_category.png}    \label{fig:output_category}}
%     \caption[]{\junjie{Top identified output format overall(across all themes).}\mao{For all the used bar charts, now the font size is too small for some word, can we adjust it?}}
%     \label{fig:output_format_oveerall}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/output_format/input_output_relationship.png}
%     \caption{\junjie{Input to output format flow (\# occurrence >=10).}}
%     \label{fig:input_output}
% \end{figure}


\subsection{RQ2: Analyzing Content and Structural Patterns in Components}
In RQ2, we aim to further analyze prompt components based on the findings from RQ1. We conduct a word-level and phrase-level analysis for each type of component in the collected prompt templates. Specifically, we examine different ways of expressing similar component content (\eg, the various ways users describe the output format as "JSON") to identify common patterns. From these variations, we identify common patterns and test their effectiveness to determine which formulations are the most reliable and impactful for writing specific components.

We perform an in-depth analysis of specific prompt components that have a significant impact on the structure consistency and instruction relevance of LLM responses, focusing on commonly used words, phrases, and formats associated with these components. Among the seven types of prompt components, we focus on two: Output Format/Style and Constraints. In direct interactions with LLMs (such as live chat), users primarily care about the relevance and correctness of the response. However, in LLM-based applications, developers are not only concerned with the response content but also with its format, as post-processing often relies on structured outputs. Ensuring a limited or predictable output format can significantly reduce errors during post-processing. Based on our observations of how LLM-based applications handle responses, we focus on Output Format/Style and Constraints due to their critical role in shaping both the response format and content, which are essential for downstream processing and application performance.

\noindent \textbf{Output Format/Style. }We analyze the output formats specified in the prompt templates across different themes. To extract these formats, we consider the most frequently occurring terms in the output descriptions of the prompt templates and map them into word clouds for each theme, as shown in Figure~\ref{fig:output_format_word_cloud}. Words in the cloud are sized proportionally to their frequency: the larger the word, the more often that output format is used within the theme.

\begin{figure}[htpb]
    \centering
    \subfloat[][Information seeking.]{
    \includegraphics[width=0.45\linewidth]{figures/output_format/word_cloud/information_seeking.png}\label{fig:format_info}}
    \hspace{0.05\linewidth}
    \subfloat[][Creative writing.]{ \includegraphics[width=0.45\linewidth]{figures/output_format/word_cloud/creative_writing.png}\label{fig:format_writing}}
    \\
    \subfloat[][Reasoning.]{ \includegraphics[width=0.45\linewidth]{figures/output_format/word_cloud/reasoning.png}\label{fig:format_reasoning}}
    \hspace{0.05\linewidth}
    \subfloat[][Coding \& Debugging.]{ \includegraphics[width=0.45\linewidth]{figures/output_format/word_cloud/coding.png}\label{fig:format_coding}}
    \caption[]{Word cloud for output format under selected themes. }
    \label{fig:output_format_word_cloud}
\end{figure}

From our analysis, certain formats like "score" and "code" emerge as highly specific to particular themes. For example, "code" is a predominant output format in the "Coding \& Debugging" tasks, often appearing as the result of tasks such as code generation, bug fixing, and code summarization. Similarly, "score" appears frequently in "Reasoning" tasks, where users provide criteria to evaluate inputs and request LLMs to generate numerical scores based on these metrics.

Across all themes, the most common output format besides standard text is JSON. JSON's structured nature makes it particularly popular, as it is easy for applications to post-process and provides a user-friendly way to organize complex information. 

\begin{figure}[htpb]
    \centering
      \includegraphics[width=\linewidth]{figures/JSON FORMAT.pdf}
    \caption{Three different JSON output formats.}
    \label{fig:json_format}
\end{figure}


To understand how developers describe JSON output formats, we extract all prompt templates that specify JSON as the output. From the data, we identify three main patterns for defining JSON output formats. As illustrated in Figure~\ref{fig:json_format}, three key components are often used in the JSON output format:
\begin{itemize}
\item \textbf{Json Output:} This explicitly defines that the output format must be in JSON.
\item \textbf{Json Attribute Name:} This specifies the attribute names to be used in the JSON output.
\item \textbf{Json Attribute Description:} This provides detailed explanations for each attribute.
\end{itemize}
The three patterns vary in their composition of these components:
\begin{itemize}
\item \textbf{Pattern 1: Json Output} – In this pattern, developers only specify that the output should be a JSON string. They may also include general guidelines about what the JSON should contain, typically described in natural language.

\item \textbf{Pattern 2: Json Output + Json Attribute Name} – Building upon Pattern 1, developers explicitly define the attribute names to be included in the JSON output by listing them, enclosed in quotes, to ensure clarity and consistency in the structure of the output.

\item \textbf{Pattern 3: Json Output + Json Attribute Name + Json Attribute Description} – This pattern extends Pattern 2 by adding detailed descriptions of each attribute. This enhances clarity and ensures that the attributes are well understood, especially in more complex outputs.
\end{itemize}

The distribution of these patterns across all observed templates is as follows: Pattern 1 (Json Output) 36.21\%, Pattern 2 (Json Output + Json Attribute Name) 19.83\%,
Pattern 3 (Json Output + Json Attribute Name + Json Attribute Description) 43.97\% of the cases. 


% To evaluate how these three patterns affect the quality of LLM-generated outputs, we select five representative prompt templates for each pattern. We then manually reformulate these templates into other patterns, resulting in 45 total prompt templates.
% We use \gptversion to generate three diverse inputs for each prompt template, and employed \llamaversion to generate outputs for the prompts.

% The evaluation is conducted using human assessments, applying two key metrics (integers from 1 to 5):
% \begin{itemize}
% \item \textit{Format} evaluates whether the generated JSON strings adhere to the format defined in the prompt and the consistency of the format across outputs derived from the same prompt template.

% \item \textit{Content} assesses the relevance of the generated content to the requirements specified by the prompt template.
% \end{itemize}

% The results presented in Table~\ref{tab:json_format}, indicate that Pattern 2 and Pattern 3 achieve high scores for "Format," whereas Pattern 1 scores significantly lower. This discrepancy is primarily due to variability in the number of attributes and their names across outputs in Pattern 1. The explicit definition of "Json Attribute Name" in Patterns 2 and 3 helps enforce a consistent output structure, thereby narrowing the generation space and preventing the extraction of irrelevant or extraneous information.

% For the "Content" score, Pattern 3 significantly outperforms the other two, indicating that the existence of detailed "Json Attribute Descriptions" enables the LLM to better understand and generate content that aligns with the user's requirements. This highlights the importance of providing attribute-level descriptions to ensure accurate and relevant output from the model.

% \input{tables/json_pattern_evaluation}

% Figure~\ref{fig:json_example} illustrates a specific example of extracting information from a tweet using three similar prompt templates, each with identical input text but differing in their JSON output format. Case 1 simply requests a JSON output with a broad description of the information needed, without explicitly defining the required fields. This results in outputs that include redundant fields like "text", "mentions", "hashtags", and "created\_at", which diverge from user expectations and introduce unnecessary information. In contrast, Case 2 specifies particular field names, such as "tweet\_id", "username", "timestamp", and "engagement", contributing to a more consistent and structured output. However, while these field names are relatively intuitive, some attributes, such as "username" and "timestamp", can have multiple interpretations. In the context of Twitter, for instance, "username" should refer to the Twitter handle, prefixed by "@", and "timestamp" should adhere to ISO 8601 format. The absence of explicit clarifications in Pattern 2 leaves room for ambiguity. Case 3 effectively addresses these ambiguities by providing clear descriptions alongside each attribute. For example, it defines "username" as "the username of the user who posted the tweet, prefixed with '@'," and specifies that "timestamp" should follow the ISO 8601 format. By explicitly detailing each field, Pattern 3 reduces interpretative flexibility, significantly enhancing both output accuracy and alignment with user expectations.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/JSON EXAMPLE.pdf}
%     \caption{An example of different json output format patterns. \chen{Anything special? Do not seem very interesting.}}
%     \label{fig:json_example}
% \end{figure}



\noindent \textbf{Constraints.} We employ the \llamaversion\ model to automatically identify different constraint types, following the classifications of constraint components established by Ross Dawson~\cite{rossdawson_prompt_elements}. Figure~\ref{fig:constraints_type} presents the distribution of the various constraint types observed in our analysis. The top three constraint types are "Exclusion" (46.0\%), "Inclusion" (35.6\%), and "Word count" (10.5\%). These categories represent the major considerations developers emphasize when constructing prompt templates. "Inclusion" directs the model to focus on specific information or details, it helps guide the model’s attention toward relevant or required content, improving the precision and relevance of the response. "Word count"  encourages the model to deliver concise responses by increasing the density of relevant information. This not only makes the output more user-friendly by eliminating unnecessary verbosity but also helps reduce API usage costs, as shorter outputs require fewer tokens and processing resources.

\begin{figure}[htpb]
    \centering
     \includegraphics[width=\linewidth]{figures/constraints_type.png}
    \caption{Relative frequency distribution of constraints type.}
    \label{fig:constraints_type}
\end{figure}

\input{tables/what_not_to_include}

Given that "Exclusion" represents nearly half of all identified constraints, we performed a more detailed analysis of this specific type. Using the same method applied in our thematic analysis—leveraging the all-mpnet-base-v2 embedding in conjunction with k-means clustering—we identified five distinct subcategories within this constraint type, as shown in Table~\ref{tab:not_include}. These subcategories provide insights into the nuances of developer intent when defining what should be excluded in prompt-generated outputs. Additionally, we list the corresponding inclusion examples to highlight the differences between exclusion and inclusion constraints.


The most critical subcategories, "accuracy and relevance" and "clarity about unknowns," serve to mitigate hallucinations, a prevalent issue in large language models (LLMs). For example, instructions like "Don't try to make up an answer" explicitly guide the LLM to avoid generating speculative or incorrect information, thereby reducing the likelihood of hallucinations. By encouraging the model to admit gaps in knowledge instead of fabricating content, developers can significantly enhance the reliability and trustworthiness of outputs.

Moreover, developers often aim to minimize unnecessary outputs, reducing redundancy in the generated content. Prompts that specify constraints like "do not generate redundant information" under the subcategory "Redundancy and Context
Adherence" are designed to optimize responses by streamlining the information, which, in turn, reduces post-processing efforts. This is especially beneficial in LLM-based applications that require strict formatting or concise answers, such as code generation tasks, customer service interactions, or technical documentation.

Another notable subcategory, "technical restriction", reflects the practical constraints imposed in specific contexts, such as database queries or API calls. Prompts in this category ensure that LLMs operate within defined technical limitations, such as using only specific column names in database queries or adhering to predefined structures. This level of precision is crucial for maintaining the correctness and efficiency of outputs in applications that demand high technical accuracy.

% We use \textit{Output Simplicity} as the evaluation metric, where:

% \begin{itemize}
% \item A score of 1 is given if the output consist solely of the JSON string, making it directly parsable by a JSON parser API.

% \item A score of 0 is given if the output include any other text besides the JSON string.
% \end{itemize}

% The result is listed in Table~\ref{tab:constarint}. "Prompt" represents the original examples from the JSON format experiment, while "Prompt with Constraint" indicates the examples where the "what not to include" constraint is applied. From the results in Table~\ref{tab:constarint}, we can observe that applying the constraint substantially improved the output. For the Prompt without constraints, the Output Simplicity score is 0.4, which means that only 40\% of the time, the output consists solely of the required JSON string, while the rest of the time, additional explanations or comments are generated. When the "what not to include" constraint are applied, the Output Simplicity score increased to 0.8, indicating that 80\% of the outputs contain only the required JSON string. In the single failed case, the output still adheres closely to the constraint but is surrounded by """json""", which is not considered redundant text. This clearly demonstrates the impact of the "what not to include" constraint in reducing redundancy and ensuring that the output adheres strictly to the required format. 

% \input{tables/constraint}


% In conclusion, understanding these constraint types and subcategories helps developers fine-tune LLM outputs, making them more aligned with user needs and reducing potential issues like hallucinations, redundancy, and technical errors. This approach not only enhances the efficiency of LLM-based systems but also supports broader applications in real-world scenarios where precision and accuracy are paramount.

\begin{tcolorbox}[colback=black!5!white,colframe=black!75!black,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm},left=0.1pt, right=0.1pt]
\textbf{Answer to RQ2:} In our analysis of the Output Format/Style component, JSON emerged as the most frequently used output format. Within those JSON format definitions, three key elements—JSON Output, JSON Attribute Name, and JSON Attribute Description—are consistently used to define output requirements. We identified three main construction patterns among these elements for structuring JSON output specifications. For the Constraints component, Exclusion was the most commonly applied constraint type, serving to limit output by excluding irrelevant content, reducing hallucinations about uncertain information, and narrowing down the types of database queries or API calls.
\end{tcolorbox}

\begin{comment}
\begin{table}[htpb]
\caption{What not to include. \chen{1. Can we also take inclusion into one column? 2. I think that we do not need cluster ID/key themes? 3. try to align the table with the corresponding main text in the same page.}}
\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{c p{3cm} p{7cm}}
\toprule
\textbf{Cluster ID} & \textbf{Key Themes} & \textbf{Representative Examples} \\
\midrule

\multicolumn{3}{c}{\textbf{Concise Output}} \\ 
\midrule

0 & Output control (what text/ code should be excluded) & 
- do not provide any other \textbf{output text or explanation}. \newline 
- if you are calling a function, only include the function call -- \textbf{no other text}. \\ 
\midrule

3 & Redundancy and context adherence & 
- \textbf{don't} give information outside the document or \textbf{repeat your findings}. \newline 
- \textbf{do not generate redundant information.} \\  \midrule

\multicolumn{3}{c}{\textbf{Accuracy Output}} \\ 
\midrule

1 & Accuracy and relevance & 
- \textbf{do not try to make up an answer.} \newline 
- \textbf{avoid adding any extraneous information.}\\  \midrule

2 & Clarity about unknowns & 
- \textbf{if you don't know the answer}, just say that you don't know, \textbf{don't try to make up an answer.} \newline 
- \textbf{if you don't know the answer}, just say you don’t know.\textbf{don't try to make up an answer.}\\
\midrule

\multicolumn{3}{c}{\textbf{Technical Restrictions}} \\  \midrule

4 & Technical restriction & 
- \textbf{never write any query other than a select}, no matter what other information is provided in this request. \newline 
- pay attention to use only the column names you can see in the tables below. Be careful to \textbf{not query for columns that do not exist.} Also, pay attention to which column is in which table. \\ 
\bottomrule

\end{tabular}
}
\label{tab:not_include}
\end{table}
\end{comment}



\subsection{RQ3: Classifying and Positioning Placeholders}
In RQ3, we analyze the types of placeholders (variables which will be replaced by input text to create a complete prompt) within prompt templates~\cite{schulhoff2024prompt}, focusing on categorizing them based on their variable names and contextual usage within the templates. Then we examine the positional distribution of placeholders across prompt templates.

\noindent \textbf{Classification of Placeholder. } Figure~\ref{fig:placeholder_type} displays the classification results of placeholders. The most prevalent categories are Metadata/Short Phrases and Knowledge Input. Metadata/Short Phrases serve as brief inputs providing essential settings or specific details, such as "language” or "username." Knowledge Input placeholders contain the main content with which the LLM directly interacts, including items like "report" or "code snippet." Additionally, the User Question placeholder captures the direct query from the end user, while Contextual Information placeholders provide supplementary background content, such as “chat history” or “background info,” offering context that supports the task without being central to it.

\begin{figure}[htpb]
    \centering
  \includegraphics[width=\linewidth]{figures/placeholder_type.png}
    \caption{Relative frequency distribution of placeholder type categorized by LLM.}
    \label{fig:placeholder_type}
\end{figure}

\noindent \textbf{Positional Distribution of Placeholder.} We analyze the positional distribution of placeholders within prompt templates, dividing each template into three sections—beginning, middle, and end—each representing one-third of the template's length. Figure~\ref{fig:placeholder_position} illustrates this distribution, in which approximately 60\% of user questions appear at the end, reflecting a common structural pattern, whereas {Knowledge Input} is more evenly distributed between the beginning and end positions. Figure~\ref{fig:placeholder_example} presents examples with varied {Knowledge Input} positions. Additionally, placeholder content length varies considerably; longer Knowledge Inputs may lead to information loss in LLMs across extended prompts. We will further investigate the impact of content length on output in RQ4.

\begin{figure}[htpb]
    \centering
  \includegraphics[width=\linewidth]{figures/placeholder_position.png}
    \caption{Frequency distribution of placeholder positional occurrences (beginning, middle, end) under different placeholder types, excluding "Others".}
    \label{fig:placeholder_position}
\end{figure}

% To analyze the effect of Knowledge Input position and length on output quality, we conduct an experiment. We randomly select three prompt templates, each containing an instruction, Knowledge Input placeholder, and User Question placeholder, and adjust the position of instructions to cover cases where they appear both before and after the Knowledge Input. Each template is filled with sample data relevant to its task, drawn from diverse sources: a medical QA dataset \cite{}, JAVA official documentation \cite{}, and a GitHub open-source project \cite{}. The medical dataset inherently includes highly similar data of varying lengths, allowing us to use these samples directly as our long, medium, and short inputs. Here, "long" is defined as content exceeding 4000 tokens, "medium" as content between 1000 and 4000 tokens, and "short" as content below 1000 tokens, based on \llamaversion's maximum sequence length of 8192 tokens. For the JAVA and GitHub data, we use the original data as long inputs and truncate them for medium and short samples, ensuring content consistency without rewriting. Each template is accompanied by a single user question crafted based on the shortest Knowledge Input sample.

% The evaluation is conducted using human assessments, applying two key metrics (integers from 1 to 5):
% \begin{itemize}
% \item \textit{Relevance to Question} evaluates whether the generated output adhere to what user want to know.

% \item \textit{Consistency to Instruction} assesses how the generated output fit to the instruction.
% \end{itemize} 

% Table \ref{tab:placeholer_length} presents the final result. Regarding the Relevance to Question metric, all three content length categories (short, medium, and long) achieved relatively high scores, demonstrating that the models maintained strong alignment with the user question at the end of prompt template across varying input lengths.

% However, in terms of Consistency to Instruction, the results reveal a notable trend: as the length of the knowledge input increases, the score gap between Pattern 1 (where the instruction precedes the knowledge input) and Pattern 2 (where the instruction follows the knowledge input) widens. Specifically, the score drops more significantly in Pattern 1 as the input length increases, with the long input scenario showing the most pronounced difference (4.44 vs. 3.00). This suggests that when the instruction is placed before the knowledge input, the model's ability to retain the instruction diminishes as the length of the input grows. In contrast, in Pattern 2, where the instruction comes after the knowledge input, the model remains more consistent in following the instruction, regardless of input length.

% This phenomenon occurs because longer knowledge inputs increase the likelihood that the model will forget or lose focus on earlier parts of the prompt, especially the instruction, if it appears at the beginning. Consequently, the consistency of the output with the instruction is weakened in those cases.

% \input{tables/placeholer_content_length}

% Figure~\ref{fig:placeholder_length} illustrates an example with a long input text. In this comparison, Pattern 1 (left) positions the instruction before the knowledge input, while Pattern 2 (right) positions the instruction after the knowledge input. In both cases, the user question remains at the end of the prompt template. The colored sections of the prompt differentiate between the instruction (red), knowledge input (green), and user question (grey). The upper portion of each side presents the filled prompt template, while the lower portion showcases the respective LLM output. In this example, the long input is a detailed description about skin cancer. Regarding the LLM outputs, both patterns provide similar responses to the user question, with the middle portion of the long description about skin cancer being reduced in both cases. However, the differences arise in how the LLM addresses the facts required by the instruction. In Pattern 1, the "curious fact" output discusses what the skin is, which, although interesting, is unrelated to the user question. Additionally, the relevant fact is missing. In contrast, Pattern 2 generates more aligned results. The "curious fact" and "relevant fact" both relate to skin cancer types, discussing where they occur (\eg, on mucous membranes) and their occurrence across various skin tones, thus providing a more relevant and comprehensive response to the instruction and user question. This suggests that placing the instruction after the knowledge input (as in Pattern 2) can lead to more accurate adherence to instructions, especially when dealing with long knowledge inputs.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/PLACEHOLDER_LENGTH.pdf}
%     \caption{A prompt template example with placeholder of different position and content length.}
%     \label{fig:placeholder_length}
% \end{figure}
\begin{figure}[htpb]
    \centering
  \includegraphics[width=\linewidth]{figures/placeholder_example.png}
    \caption{Examples of prompt templates with different Knowledge Input positions.}
    \label{fig:placeholder_example}
\end{figure}

\begin{tcolorbox}[colback=black!5!white,colframe=black!75!black,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm},left=0.1pt, right=0.1pt]
\textbf{Answer to RQ3:} Placeholder analysis identifies Metadata/Short Phrases and Knowledge Input as the most common categories. Metadata captures brief settings details like "language," while Knowledge Input contains the main content (\eg, "code snippet") that the LLM processes. User Questions typically appear at the end of templates (60\%), while Knowledge Inputs are evenly split between the beginning and end. Placeholder content length also plays a role, with extended Knowledge Inputs sometimes affecting LLM performance, as explored further in RQ4.
\end{tcolorbox}

\subsection{RQ4: Evaluating Patterns through Sample Testing}

% \mao{Dos and Don'ts} Dos: 1. Json Output Format and 2. Positional Relationship between Placeholder and Instruction

% Don'ts: 1. Exclusion Constraint for Conciseness


In RQ4, we explore how prompt templates influence LLM instruction-following abilities, focusing on two key dimensions: Content-Following and Format-Following. Content-Following ensures the semantic accuracy of outputs with respect to user-defined goals, critical for all LLM usage contexts. Format-Following, on the other hand, guarantees adherence to specified structural or syntactical requirements, a factor underexplored in prior research but vital for \llmapp~\cite{xia2024fofo}.
To address these aspects, we test patterns identified in earlier research questions, concentrating on JSON Output Format, Exclusion Constraint for Output, and Variance of Placeholder. Representative prompt templates are selected randomly, populated with sample data using the \gptversion\ model and existing datasets, and used to generate outputs via \llamaversion\ and \gptversion\ models. These outputs are then evaluated on key metrics through human assessment.

\noindent \textbf{Json Output Format. } To investigate the effect of different JSON output patterns, we test three identified patterns: Pattern 1 (JSON Output), Pattern 2 (JSON Output + JSON Attribute Name), and Pattern 3 (JSON Output + JSON Attribute Name + JSON Attribute Description). Five representative templates are selected for each pattern, yielding a total of 45 templates after reformatting them to fit all patterns.

For testing, three diverse input instances are generated per template using \gptversion\ model. Both \llamaversion\ and \gptversion\ models produce corresponding JSON outputs, evaluated solely on the JSON object portion, excluding any explanatory text. Two metrics, rated on a 1-to-5 scale, are used for evaluation:
%For testing, we use \gptversion\ to generate three diverse input instances per template and \llamaversion\ to produce corresponding JSON outputs, focusing solely on the JSON object portion and ignoring any additional explanatory text. The output quality is then assessed based on two key metrics, each rated from 1 to 5:
\begin{itemize}
%\item \textit{Format Consistency} measures the extent to which the generated JSON strings align with the prompt-defined format and maintain structural consistency across outputs for the same template.
\item \textit{Format Following: } Measures the consistency of generated JSON strings with the defined format, including attribute count, names, and structural uniformity across outputs.

%\item \textit{Instruction Relevance} evaluates the alignment of generated content with the specified requirements in the prompt template.
\item \textit{Content Following: } Assesses the alignment of generated content with the user-defined intent in the prompt template.
\end{itemize}

\input{tables/json_pattern_evaluation}

As shown in Table~\ref{tab:json_format}, both models exhibit similar trends, with Pattern 3 achieving the highest scores across metrics and models. In Format-Following, Patterns 2 and 3 outperform Pattern 1, which scores lower due to inconsistencies in attribute count and naming, stemming from its lack of explicit definitions. Patterns 2 and 3 mitigate these issues through explicit "JSON Attribute Names," ensuring greater structural consistency.

For Content-Following, Pattern 3 achieves the highest scores, with \llamaversion\ reaching 4.47 (+0.45) and \gptversion\ reaching 4.53 (+0.23), suggesting that detailed "JSON Attribute Descriptions" enhance the model's ability to generate content that aligns closely with user requirements. These findings underscore the value of attribute-level detail in improving both precision and semantic adherence.


%As shown in Table~\ref{tab:json_format}, Patterns 2 and 3 score highly in "Format Consistency", while Pattern 1 scores significantly lower. This lower score in Pattern 1 is mainly due to variability in attribute count and naming across outputs, as it lacks explicit definitions. Patterns 2 and 3, by specifying "JSON Attribute Name", ensure a stable output structure, minimizing irrelevant or extra details.

%For "Instruction Relevance", Pattern 3 achieves the highest scores, indicating that the inclusion of detailed "JSON Attribute Descriptions" helps the model better understand and produce content that accurately meets the user’s requirements. These findings underscore the importance of attribute-level detail in improving both the relevance and precision of LLM outputs.

\begin{figure}[htpb]
    \centering
     \includegraphics[width=\linewidth]{figures/JSON EXAMPLE.pdf}
    \caption{An output example of different json output format patterns.}
    \label{fig:json_example}
\end{figure}

Figure~\ref{fig:json_example} illustrates a specific example of extracting information from a tweet using three similar prompt templates, each with identical input text but differing in their JSON output format. Case 1 simply requests a JSON output with a broad description of the information needed, without explicitly defining the required fields. This results in outputs that include redundant fields like "text", "mentions", "hashtags", and "created\_at", which diverge from user expectations and introduce unnecessary information. In contrast, Case 2 specifies particular field names, such as "tweet\_id", "username", "timestamp", and "engagement", contributing to a more consistent and structured output. However, while these field names are relatively intuitive, some attributes, such as "username" and "timestamp", can have multiple interpretations. In the context of Twitter, for instance, "username" should refer to the Twitter handle, prefixed by "@", and "timestamp" should adhere to ISO 8601 format. The absence of explicit clarifications in Pattern 2 leaves room for ambiguity. Case 3 effectively addresses these ambiguities by providing clear descriptions alongside each attribute. For example, it defines "username" as "the username of the user who posted the tweet, prefixed with '@'," and specifies that "timestamp" should follow the ISO 8601 format. By explicitly detailing each field, Pattern 3 reduces interpretation ambiguities, significantly enhancing both output accuracy and alignment with user expectations.


\begin{tcolorbox}[colback=black!5!white,colframe=black!75!black,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm},left=0.1pt, right=0.1pt]
  \textbf{Findings 1: } When generating LLM outputs in JSON format, explicit JSON Attribute Names (Patterns 2 and 3) enhance format consistency by ensuring structured and uniform outputs. Additionally, detailed Attribute Descriptions (Pattern 3) further refine content-following, reducing ambiguity and enabling outputs to better align with user-defined requirements.
\end{tcolorbox}


\noindent \textbf{Exclusion Constraint for Output. } Explicitly defined JSON output formats represent "Do" instructions for shaping outputs. However, developers also employ "Don't" instructions, such as exclusion constraints, to ensure concise outputs. Building on insights from RQ2, we evaluate the effectiveness of exclusion constraints in reducing redundancy by refining outputs to focus solely on JSON objects. To test this, we use five templates from the JSON Output Pattern 3 experiment, each populated with three sample instances used before. Without exclusion constraints, LLM outputs often include redundant explanatory text alongside the JSON object, deviating from the intended format. To mitigate this, we apply the exclusion constraint: "Do not provide any other output text beyond the JSON string," placed before the JSON format definition per patterns observed in RQ1.

For evaluation, we define the metric \textit{Format Following} as follows:

\begin{itemize}
\item \textbf{Score of 1: } Output consists solely of the JSON string, ready for direct parsing.

\item \textbf{Score of 0: } Output contains extraneous text outside the JSON string.
\end{itemize}

Results highlight the impact of the exclusion constraint. For \llamaversion\ model, the original prompts yield a Format Following rate of 40\% (only JSON string in 40\% of outputs). The constraint raises this rate to 100\%, demonstrating improved adherence. 
In 16.67\% of cases, the output is enclosed in """json""" without any other explanation text, which we do not consider redundant.
\gptversion\ performs better with the original prompts, achieving an 86.67\% adherence rate, further increasing to 100\% with the exclusion constraint applied. These findings underline the exclusion constraint's value in improving clarity, reducing redundancy, and ensuring strict adherence to output format requirements.

% \input{tables/constraint}
\begin{tcolorbox}[colback=black!5!white,colframe=black!75!black,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm},left=0.1pt, right=0.1pt]
  \textbf{Findings 2: } Using only JSON format definitions is insufficient to fully prevent extraneous explanations or comments. Combining "Do" instructions, such as explicit output format definitions, with "Don't" instructions, like exclusion constraints, significantly reduces redundancy while maintaining high output consistency in LLM-generated content.
\end{tcolorbox}



\noindent \textbf{Variance of Placeholder. } Placeholders play a crucial role in prompt templates, and their position relative to other components, along with their variable content length, significantly impacts LLM outputs. In this experiment, we focus on a retrieval-augmented generation (RAG)-style task where users pose questions, external knowledge is provided as input, and developers define instruction (\eg, directive, constraint, output format) to process the dynamic input. To examine the impact of the \{Knowledge Input\} placeholder's position (equally distributed at the beginning and end of the prompt as identified in RQ3) and content length on output quality, we test two prompt configurations: Pattern 1, where the task intent part of instruction precedes the knowledge input, and Pattern 2, where it follows. In both configurations, the \{User Question\} placeholder remains at the end, as observed in RQ3. The prompt templates are populated with data from diverse sources, including a medical QA dataset~\cite{ben2019question}, Java documentation~\cite{jdk22}, and GitHub projects~\cite{transformer}, with input lengths categorized as short (<1000 tokens), medium (1000–4000 tokens), and long (>4000 tokens) based on \llamaversion\ API's sequence length of 8192 tokens. Although \gptversion\ supports a larger context window, the same inputs are used for consistency.

Evaluation is conducted using two human-assessed metrics on a 1–5 scale:
\begin{itemize}
\item \textit{Content Following (Question): } Alignment with the user question.

\item \textit{Content Following (Task Intent): } Adherence to the task intent of instruction, including directive, constraint and output format.
\end{itemize} 

Table \ref{tab:placeholer_length} shows the results. Both models exhibit high scores for Content Following (Question) across all input lengths and patterns, reflecting consistent alignment with user queries at the end of the prompt template. However, the scores for Content Following (Task Intent) highlight a distinct trend: as knowledge input length increases, Pattern 1 suffers a more significant performance drop compared to Pattern 2. For instance, with long inputs, the task intent adherence score decreases from 4.44 to 3.17 for \llamaversion\ and from 4.56 to 3.67 for \gptversion\ in Pattern 1, while Pattern 2 maintains strong performance (4.89 for LLaMA and 4.34 for GPT). This suggests that placing the task intent of instruction before the knowledge input (Pattern 1) increases the likelihood of forgetting or misalignment as input length grows. Conversely, Pattern 2 mitigates this issue, maintaining robust task intent adherence even with long inputs. The observed phenomenon aligns with the hypothesis that longer inputs lead to information decay, affecting earlier prompt components.

\input{tables/placeholer_content_length}

\begin{figure}[htpb]
    \centering
  \includegraphics[width=\linewidth]{figures/PLACEHOLDER_LENGTH.pdf}
    \caption{A prompt template example with placeholders of different positions and content length.}
    \label{fig:placeholder_length}
\end{figure}

Figure~\ref{fig:placeholder_length} illustrates an example with a long input text. In this comparison, Pattern 1 (left) positions the instruction before the knowledge input, while Pattern 2 (right) positions the instruction after the knowledge input. In both cases, the user question remains at the end of the prompt template. The colored sections of the prompt differentiate between the instruction (red), knowledge input (green), and user question (grey). The upper portion of each side presents the filled prompt template, while the lower portion showcases the respective LLM output. In this example, the long input is a detailed description about skin cancer. Regarding the LLM outputs, both patterns provide similar responses to the user question, with the middle portion of the long description about skin cancer being reduced in both cases. However, the differences arise in how the LLM addresses the facts required by the instruction. In Pattern 1, the "curious fact" output discusses what the skin is, which, although interesting, is unrelated to the user question. Additionally, the relevant fact is missing. In contrast, Pattern 2 generates more aligned results. The "curious fact" and "relevant fact" both relate to skin cancer types, discussing where they occur (\eg, on mucous membranes) and their occurrence across various skin tones, thus providing a more relevant and comprehensive response to the instruction and user question.


\begin{tcolorbox}[colback=black!5!white,colframe=black!75!black,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm},left=0.1pt, right=0.1pt]
  \textbf{Findings 3: } Longer knowledge inputs increase the likelihood of diminished focus on earlier prompt elements. Positioning the task intent of instruction and user question after the knowledge input (\{Knowledge Input\} → Task Intent → \{User Question\}) enhances output consistency and mitigates information decay in LLM responses, particularly when processing prompt templates with highly variable input lengths in LLM applications.
\end{tcolorbox}

\begin{tcolorbox}[colback=black!5!white,colframe=black!75!black,before upper=\vspace{-.2cm},after upper=\vspace{-.2cm},left=0.1pt, right=0.1pt]
\textbf{Answer to RQ4:} To address RQ4, we reformulate randomly selected prompt templates by modifying their components or rearranging component positions based on findings from RQ1. This allows us to systematically evaluate the impact of JSON output format patterns and constraints (identified in RQ2) on LLMs' format-following and content-following capabilities. Additionally, we investigate how the position and content length of highly variable placeholders influence output alignment with both user questions and developer-defined instructions in RAG-like tasks. Through this analysis, we identify optimal prompt patterns that maximize both format-following and content-following performance in LLM applications.
% \junjie{Specific prompt template patterns influence the format- and context-following dimensions. The explicitly defined JSON Attribute Name and Attribute Description combined with the exclusion constraints ensures format-following, resulting in well-structured pure JSON output. Additionally, placing the \{Knowledge Input\} before the instruction consistently improves context following.}
\end{tcolorbox}



\subsection{Implication}
Our research offers actionable insights into prompt engineering for various parties:

\noindent \textbf{Large Model API Providers. } Large model API providers could streamline API access by simplifying prompt design.

\textit{Pre-defined Prompt Templates. }To ease the challenges developers face in designing effective prompts for applications using LLMs, pre-defined templates can provide substantial support. As highlighted in our RQ1 findings, API providers could offer templates based on pre-defined task themes. After developers select a task theme, the provider can supply a marked example template, identifying each component clearly. By clicking on components, developers can view commonly used content for reference, as noted in RQ2. Through theme-based classification of prompt data, providers can further refine templates, promoting reusable component arrangements and content.

\textit{Guidance on Prompt Caching. }Effective prompt caching can significantly reduce model latency and optimize computing resources, yet determining which prompt components to cache is often left to developers. Based on the general prompt structure patterns observed in RQ1, API providers could suggest standardized templates where component placement is consistent. This allows for increased reuse of components by maintaining stable attention states for reusable elements. Additionally, as highlighted in RQ2, providers could pre-cache frequently occurring phrases within specific components, particularly in Output Format or Constraints, ensuring that users benefit from pre-defined, reusable elements that can streamline the prompt construction process and further enhance caching efficiency.

\textit{Automated Template Evaluation Tools.} Building on insights from RQ4, LLM API providers could develop automated evaluation tools to streamline prompt template testing for \llmapp\ developers. These tools should enable comparison of outputs from different template patterns using the same inputs, helping identify optimal templates efficiently. Additionally, features like model version comparison and prompt template history tracking could be incorporated to enhance usability. Such tools would not only save time but also empower developers to refine templates and ensure consistent, instruction-following outputs in their applications.



\noindent \textbf{\llmapp\ Developers. } \llmapp\ developers can ensure high-quality outputs by focusing on prompt template testing and regular maintenance.

\textit{Testing Prompt Templates Pre-Deployment. } Ensuring consistent performance of prompt templates across diverse tasks and user inputs is crucial but can be labor-intensive. Findings from RQ4 suggest developers can utilize an additional LLM to generate varied sample inputs, simulating real-world scenarios and reducing manual effort. Moreover, insights from RQ2 and RQ3 highlight the importance of examining key components—such as Instruction, Output Format, and Constraints—for their impact on output quality. For example, when testing prompts for structured JSON outputs, developers should ensure compliance with specified formats and constraints like exclusion rules. Evaluating each component's influence on consistency and adherence to instructions allows developers to pinpoint weaknesses and refine prompts for better adaptability and reliability in handling diverse inputs.

\textit{Prompt Templates Maintenance and Update. } To enhance user experience, prompt templates should evolve based on user input patterns and feedback. By analyzing typical input lengths and content types, developers can refine placeholders effectively. For instance, if inputs are frequently long (as noted in RQ4), key information might be overlooked. Adjusting component positions in the prompt can mitigate this issue. Additionally, the granularity of placeholders should align with actual usage scenarios. For example, if users combine background and analysis in their inputs, separating these into distinct placeholders improves clarity. Incorporating metadata placeholders, such as \{output\_format\}, can further support diverse user requirements for alternative output structures.


% This research provides new insights to address key challenges in prompt template design, testing, and optimization, helping to establish a robust framework that developers can follow in the whole prompt template development lifecycle.

% \noindent \textbf{Prompt Template design. } A primary challenge in prompt template design is the difficulty developers face in organizing various prompt components effectively to meet user requirements. While developers often have a clear understanding of what information needs to be included to describe the user requirement, they lack guidance on the optimal positioning of these components within the template. 

% \noindent \textbf{Prompt Template Testing. } 
% Effective testing of prompt templates is essential to ensure they perform consistently and meet diverse user needs. However, evaluating prompt templates can be labor-intensive, especially if manual testing is used for a wide range of inputs and scenarios. Our research offers a solution by suggesting that developers can leverage another powerful LLM to generate sample inputs for testing purposes. By using an auxiliary LLM to produce varied test inputs, developers can simulate real-world scenarios and stress-test the template without requiring extensive manual input.
% During the evaluation, our findings indicate the importance of identifying and analyzing different components within the prompt, especially those with a high impact on output quality, such as Instruction, Output Format, and Constraints. For instance, in a prompt designed for generating structured JSON output, it’s crucial to verify that the output adheres to the specified Output Format while respecting constraints set by the Exclusion parameter. Evaluators should also assess how well the LLM adheres to instructions and whether the generated outputs remain consistent across varying inputs. By systematically examining each component’s contribution to the final output, developers can identify weaknesses or areas where the prompt might fail under specific conditions.

% \noindent \textbf{Prompt Template Improvement. } 
% Once a prompt template is created, a significant challenge lies in understanding why certain LLM outputs may not meet user expectations and identifying specific areas for refinement within the template. Currently, it can be difficult for developers to diagnose which part of the prompt is causing issues in the output, such as irrelevance with the user requirement or inconsistency with the intended format. 
% % Our research highlights several key components—such as JSON Output, Attribute Name, and Attribute Description for structured outputs—that play crucial roles in maintaining structural consistency and aligning with user requirements.
% % By examining the impact of these components, developers can pinpoint where refinement is needed based on user feedback. For example, if an output consistently includes irrelevant information despite the prompt specifications, refining the Exclusion Constraint component (e.g., "Do not include any information outside the JSON structure") can help narrow down the output. Furthermore, components such as Instruction and Output Format have been shown to significantly influence the quality of responses; developers can adjust these components to improve relevance and clarity. If users report dissatisfaction with response relevance, adjustments to the Output Format specifications or providing a clearer Instruction could help in aligning output with user expectations. This targeted approach to refinement based on identified component roles streamlines debugging, making it easier for developers to achieve consistent, high-quality results from their templates.



% The insights from our research have meaningful implications for advancing the accuracy and stability of outputs in future LLM-based applications, specifically addressing challenges like information relevance, output consistency, and alignment of responses with user expectations:

% \begin{itemize}
% \item[1)] \textbf{Retrieval-Augmented Generation (RAG) Systems:} RAG systems rely on user queries to identify and integrate relevant information from multiple documents. Our findings from RQ3, which examine placeholder positioning and input length, are particularly relevant to these systems. The research suggests that placing the Knowledge Input (i.e., the retrieved documents) before the User Question and Instruction components can improve output alignment with user needs, particularly when handling lengthy inputs. This order enables the model to prioritize the question and instructions, reducing the risk of distraction by extensive context and enhancing response relevance. For example, in a customer support application that retrieves information from various product manuals, positioning the user’s query and the system instructions after the knowledge input allows the model to focus more directly on user needs and system requirements, thereby improving response accuracy and relevance.
% \item[2)] \textbf{Autonomous Agent Systems}: Autonomous agent systems, often designed for complex, multi-step tasks, can also benefit from the findings in RQ1 and RQ2. These systems require prompts with diverse components and constraints to handle complex user requests effectively. Insights from RQ1 on prompt component organization help developers arrange different components to maximize interpretability and output accuracy. Additionally, findings from RQ2 on clear output format definitions and constraints promote consistency and precision in agent responses, especially in tasks with multi-step interactions and specific response formats. For instance, an agent generating financial reports can benefit from predefined JSON output formats for each data entry, which reduces errors across each stage of interaction. Applying explicit constraints, such as "return only numerical data without additional explanations" ensures that the agent adheres to strict data requirements, reducing variability and enhancing system reliability in data-sensitive contexts.

% \end{itemize}

% These findings highlight actionable strategies for improving LLM-based applications by refining prompt templates, ultimately ensuring more accurate, relevant, and consistent outputs in response to complex user tasks.

==> sections/Conclusion.tex <==
\section{Conclusion}

This paper provides an in-depth examination of prompt template structure and composition in LLM-powered applications, analyzing how developers design these templates to optimize model outputs. We constructed a dataset of prompt templates from open-source projects on GitHub, categorizing them into thematic groups and identifying common structural components. Through LLM-assisted and human-verified analysis, we examined co-occurrence patterns to identify typical positional relationships within templates.

We further analyzed the language and structure of each component, revealing commonly used terms and organizational patterns and assessing their influence on output quality through real-world testing. Additionally, we examined placeholders within prompt templates, exploring placeholder categories and variations in placement and input length. Finally, we conducted template testing to evaluate the influence of different structural patterns on the instruction-following performance of LLM response. Our findings offer foundational insights for prompt engineering, guiding the design of robust templates that enhance the accuracy and reliability of LLM outputs across various applications.

==> sections/Introduction.tex <==
\section{Introduction}
\chen{find one paper using promptset data, working on prompt evolution~\cite{tafreshipour2024prompting} which is recently accepted on MSR'25, please read it and learn from it, also cite it in the implication part or related work part. This may be the most related work.}
Large Language Models (LLMs), such as GPT-4~\cite{achiam2023gpt} and LLaMA~\cite{touvron2023llama}, have exhibited exceptional capabilities in comprehending and generating text. This versatility has introduced a new paradigm of interaction between humans and AI, where users express their requirements (\eg, task instructions, output format, or tone) through natural language prompts. The LLMs then generate outputs in accordance with these specifications. Although large models have significantly lowered the barrier to using AI for general users, crafting clear and effective prompts remains a complex task~\cite{Desmond2024ExploringPE, ZamfirescuPereira2023WhyJC}. This challenge stems from the limited understanding of how LLMs process input information and the fact that even minor variations in prompts can lead to substantial changes in model performance~\cite{salinas2024butterfly, sclar2023quantifying}.



\begin{comment}
\end{comment}
To address these challenges, numerous \llmapp, which refers to the type of software that uses LLMs as one of its building
blocks, have been developed~\cite{zhao2024llm, hou2024security}. 
\llmapp\ enhances traditional software usability by integrating the comprehension and generation capabilities of LLMs. 
These applications allow users to perform complex tasks, such as virtual assistant~\cite{alexa} or travel planning~\cite{gundawar2024robust}, through intuitive interfaces that require minimal prompt engineering skills.
%\mao{Instead of users crafting detailed prompts, developers create prompt templates, which are functions containing one or more variables that will be replaced with user-specific inputs (often text) to form a complete prompt~\cite{schulhoff2024prompt}.
Unlike traditional software development that involves full-stack implementation, \llmapp\ intends to build a low-code development paradigm with powerful LLMs serving all user interactions, and developers will develop light-weight prompt templates, which are predefined prompt structures designed to simplify and standardize user interactions with LLMs~\cite{gorissen2024survey, schulhoff2024prompt}.
Prompt templates function as critical artifacts in \llmapp, as they abstract the complexity of crafting effective prompts away from users, bridging user intent and machine response.
By providing a consistent structure, prompt templates help users articulate their requirements more effectively, ensuring that the LLM understands and responds appropriately even in specialized domains, such as document analysis~\cite{wang2024knowledge}, creative content generation~\cite{chen2024benchmarking}, and code synthesis~\cite{guo2024stop}. 
Figure~\ref{fig:prompt_template_example} illustrates a prompt template for a music recommendation system. The template defines the model’s role, provides directives (song suggestion), and specifies constraints such as returning results in a predefined JSON format. The \{user\_requirement\} placeholder accommodates diverse user inputs like "light music for bedtime" or "a song with a summer feel describing ... life in ...". This template ensures output relevance and consistency while maintaining an intuitive and user-friendly interaction.




\begin{figure}[htpb]
    \centering
      \includegraphics[width=\linewidth]{figures/PROMPT TEMPLATE EXAMPLE.pdf}
    \caption{An example of prompt template.}
    \label{fig:prompt_template_example}
\end{figure}

%\chen{This part is too abstract and requests in-depth analysis. Note that LLMapp is also one kind of software, and many techniques are well established in SE such as software development, testing, maintenance, etc, and why not apply them to prompts LLMapp? No, prompt template is not like code template and existing methods fall short in many aspects, (tell more details), and that is why we need a comprehensive analysis of existing prompt templates to further understand the opportunity and challenges.}
%\mao{Despite the maturity of testing and bug detection techniques in traditional software engineering, these methods offer limited benefits for FMware applications.  Conventional testing approaches, such as code-based and functionality-based testing, depend on access to core code logic or consistent outputs for identical inputs. However, the underlying mechanisms of foundation models remain largely opaque, preventing code-based testing. Additionally, functionality-based testing is challenging due to the inherent variability in model responses to the same prompt, along with the difficulty in defining expected outputs. For bug detection, techniques that rely on detailed error reports (\eg, specific exceptions or error locations in the code) are inadequate for VMware, where issues often manifest as subtle misalignments with user requirements. Identifying and refining the problematic parts of complex prompt templates is thus a non-trivial task. ~\junjie{Clear bug descriptions have shown improvements in bug localization performance~\cite{Saha2024TowardTA}, suggesting that well-structured prompts could enhance FMware performance. }Given these limitations, research into effective prompt template design is essential to ensure the reliability and performance of FMware applications, as prompt templates serve as a critical layer for aligning model outputs with application goals.} \chen{Always need \textbf{references} to support your claim. Note that we need to make our research papers convincing.}
Despite the growing significance of prompt templates in the \llmapp\ ecosystem, a systematic understanding of their structure, composition, and effectiveness remains underdeveloped. 
Unlike traditional software development, which is deterministic and relies on well-defined code~\cite{li2023cctest, holter2024abstract, yuan2024evaluating}, \llmapps\ introduce variability in outputs, challenging software engineers to design prompts that ensure reliability, maintainability, and performance.
This gap presents significant implications for software engineering. Just as requirements specifications guide traditional development, prompt templates encapsulate intent for LLMs, influencing system behavior and output quality.
The software engineering research community has yet to develop a cohesive framework for understanding how prompt templates are constructed, which components contribute most effectively to model performance, and how variations in content within the same placeholder affect LLMs' ability to follow instructions.
Addressing this gap is critical to designing consistently high-performing prompt templates for \llmapps, drawing parallels to established design patterns in software engineering practices~\cite{white2023prompt}.
Therefore, we propose the following research questions:
\begin{itemize}
    \item RQ1: What are the common task themes and constituent components in prompt templates?
    \item RQ2: What specific words and phrases are frequently used in different components, and are there common construction patterns?
    \item RQ3: How do placeholders vary in terms of types and positions within prompt templates?
    \item RQ4: How do different construction patterns in prompt templates influence LLMs' instruction-following abilities?
\end{itemize}

In this paper, we analyze prompt templates used in LLM-based applications, focusing on their thematic tasks, components, reusable content, and placeholder types and positions. Using a publicly available prompt dataset~\cite{pister2024promptset}, we pre-process it and classify templates by themes and constituent components through LLM-based analysis and manual verification. We identify general component arrangement patterns, uncover two primary positional patterns, and highlight JSON as the most common output format. Explicitly defined JSON attributes with descriptions improve format consistency and semantic relevance, while constraints reduce output redundancy. For placeholders, we categorize four main types and analyze their positions. Based on the identified patterns, we conduct sample testing with randomly selected templates to evaluate how different patterns influence LLM instruction-following abilities and identify optimal patterns.

Our contributions are summarized as follows:
\begin{itemize}
    \item To the best of our knowledge, this is the first study analyzing real-world prompt templates in \llmapp.
    \item We identify and categorize key components and placeholders within prompt templates, offering insights into effective prompt template design practices.
    \item Through sample testing, we demonstrate that well-structured prompt templates and specific composition patterns can significantly improve the instruction-following abilities of LLMs.
\end{itemize}


==> sections/Methodology.tex <==
\section{Methodology}

\subsection{Overview}
Figure~\ref{fig:overview} shows the main framework of our method. The pipeline involves three main phases: data collection, prompt template analysis, and prompt template testing.

\begin{figure}[htpb]
 \centering
  \includegraphics[width=\linewidth]{figures/OVERVIEW.pdf}
  \caption{An illustration of the main pipeline.}
  \label{fig:overview}
\end{figure}

In the data collection phase, we preprocess a publicly available dataset of prompts~\cite{pister2024promptset} extracted from GitHub projects, tagging each entry with metadata such as repository stars and last update time. We then filter this dataset to retain a subset of representative prompt templates for analysis.

In the prompt template analysis phase, we define categories for prompt themes, components, and placeholders. With these categories, we leverage an LLM to classify prompt themes and identify components and placeholders within each template. We then perform statistical analysis to examine the distribution and positioning of these components, identifying co-occurrence patterns within templates.

In the prompt template testing phase, we randomly select templates from various identified patterns to assess how these patterns influence the instruction-following of LLM output.

Human evaluations are conducted to assess the accuracy of our theme classification, component identification, and placeholder identification results, as well as the instruction-following quality of LLM output for sample data during prompt template testing. Two participants, a postgraduate and a PhD student specializing in software engineering, each with over a year of programming experience in \llmapp, conduct the human evaluation.
For classification and analysis tasks, participants review the LLM-generated results on theme classification, component identification, and placeholder identification for each sample. If any result is regarded as incorrect, they provide their own corrections. For prompt template testing, they score the LLM output based on predefined quality metrics; if their scores differ by more than 20\% of the total possible score, they discuss to determine a final score. The final score is then taken as the average of both participants' evaluations.

The following sections provide detailed explanations of each phase.


\subsection{Data Collection}

% \subsection{Data Collection}
% \begin{figure}
%  \centering
% \includegraphics[width=0.95\textwidth]{figures/DATA_COLLECTION.pdf}
%   \caption{Data processing pipeline.}
%   \label{fig:DataProcessingPipeline}
% \end{figure}

We construct our dataset using PromptSet~\cite{pister2024promptset}, a collection of prompts extracted from LLM-powered applications. The prompts in PromptSet are gathered from open-source projects on GitHub as of January 10, 2024. These projects span varying levels of complexity and usage, such as student assignments, personal demos, and community-driven initiatives, resulting in significant variability in prompt quality. To ensure high-quality data, we develop a processing pipeline that assigns quality metrics to each prompt and automatically filters out lower-quality prompts.

The data collection pipeline for our study begins with selecting non-empty English prompts from the PromptSet dataset, resulting in 14,834 records. For each associated GitHub repository, we retrieve metadata such as \textit{star count} and \textit{latest update time} to evaluate popularity and activity~\cite{weber2014makes, cosentino2016findings}. We then filter this set to include only repositories with at least five stars and recent updates within the past year, resulting in 2,888 records across 1,525 repositories. Next, we separate multi-prompt records into individual entries, resulting in 5,816 prompts, and then remove duplicates to obtain 4,540 unique prompts. To enhance data quality, we exclude prompts shorter than five tokens\cite{spacy2}, narrowing the dataset to 4,210 unique entries. Using the \llamaversion\ model, we extract 2,163 distinct prompt templates, guided by a clear definition from Schulhoff\etal~\cite{schulhoff2024prompt} and several illustrative prompt template examples.

\subsection{Prompt Template Analysis}
In this phase, we leverage \llamaversion\ to classify prompt themes and identify components and placeholders within each template.

\noindent \textbf{Theme Classification. } To guide prompt design for varied application needs, we categorize the collected prompts by identifying the specific task theme each prompt addresses.
We apply the prompt designed by Xu \etal~\cite{xu2024magpie}, modifying the output format to generate a single primary theme tag instead of the multiple applicable tags originally suggested. The definition of predefined task categories is displayed in Table~\ref{tab:task_tags}.

\input{tables/predifined_theme}
\begin{comment}
\begin{figure}[htpb]
    \centering
    \fbox{
    \parbox{0.95\textwidth}{
        \textbf{\# Instruction}
        \newline
        Please label the task tags for the user query.
        \newline
        \newline
        \textbf{\#\# User Query}
        \newline
        \textit{`<insert user query here>`}
        \newline
        \newline
        \textbf{\#\# Tagging the user input}
        \newline
        Please label the task tags for the user query. You will need to analyze the user query and select the most relevant task tag from the list below.
        \newline
        \newline
            all\_task\_tags=[
         \newline
        \textcolor{TUMAccentBlue}{ "Information seeking"}, \# Users ask for specific information or facts about various topics.
         \newline
          \textcolor{TUMAccentBlue}{"Reasoning"}, \# Queries require logical thinking, problem-solving, or processing of complex ideas.\newline
          \textcolor{TUMAccentBlue}{"Planning"}, \# Users need assistance in creating plans or strategies for activities and projects.\newline
          \textcolor{TUMAccentBlue}{"Editing"}, \# Involves editing, rephrasing, proofreading, or other tasks related to the composition of general written content.\newline
          \textcolor{TUMAccentBlue}{"Coding \& Debugging"}, \# Users seek help with writing, reviewing, or fixing code in programming.\newline
         \textcolor{TUMAccentBlue}{"Math"}, \# Queries related to mathematical concepts, problems, and calculations.
         \newline
         \textcolor{TUMAccentBlue}{"Role playing"}, \# Users engage in scenarios requiring ChatGPT to adopt a character or persona. 
         \newline\textcolor{TUMAccentBlue}{"Data analysis"}, \# Requests involve interpreting data, statistics, or performing analytical tasks. 
         \newline\textcolor{TUMAccentBlue}{"Creative writing"}, \# Users seek assistance with crafting stories, poems, or other creative texts.
         \newline\textcolor{TUMAccentBlue}{"Advice seeking"}, \# Users ask for recommendations or guidance on various personal or professional issues. 
         \newline\textcolor{TUMAccentBlue}{"Brainstorming"}, \# Involves generating ideas, creative thinking, or exploring possibilities. \newline\textcolor{TUMAccentBlue}{"Others"} \# Any queries that do not fit into the above categories or are of a miscellaneous nature.
         ]
        \newline
        \newline
        \textbf{\#\# Output Format:}
        \newline
        Note that you can only select a single primary tag.
        \newline
        Now, please output your tags below in a json format by filling in the placeholders in <...>:
        \newline
        '''
        \newline
        \{\{
        \newline
        \hspace*{2em}"primary\_tag": "<primary tag>"
        \newline
        \}\}
        \newline
        '''
    }
    }
    \caption{Prompts used in method 3. \chen{Too far from the text, and please try to align it with the text. BTW, a table of those tasks is enough, rather than a long prompt...}}
    \label{fig:prompt_method3}
\end{figure}
\end{comment}
To evaluate the classification performance, we randomly sample 5\% of the data from each theme category produced by each method. We then combine these samples, removing duplicates, to create a dataset for human evaluation of classification accuracy. Our method achieves a classification accuracy of 70\%.

\noindent \textbf{Prompt Component Analysis. } In this step, we first aim to define a comprehensive list of common prompt components. To identify these components, we analyze guidelines on prompt writing from popular prompt engineering frameworks and AI service platforms. Specifically, we extract prompt component definitions from Google Cloud's guide documentation~\cite{GoogleCloud}, the Elavis Saravia framework~\cite{saravia2022prompt}, the CRISPE framework~\cite{ChatGPT3FreePromptList}, and the LangGPT framework~\cite{Wang2024LangGPTRS}. To construct a unified list of prompt components, we merge similar components identified across these guidelines. For example, components such as Profile, Capacity, Role, and Persona all relate to defining the model's behavior or identity, so we combine them into a single component named "Profile/Role". As shown in Table~\ref{tab:merge}, the merged components and their definitions are presented in the last two columns.

% \junjie{The first step we need to take is to create a comprehensive list of prompt elements. In this step, similar elements will be merged. For example, the elements named profile, capacity and role and persona are all related to who the model acts as. Therefore, we merged them into a single element named "profile/role". As shown in Table~\ref{tab:merge}, the merged elements are listed in the last column. Compared with the common components included in a prompt summarized by Schulhoff et al., our merged element list includes basically all the elements mentioned in their study, ensuring comprehensive coverage.}

\begin{comment}
\begin{table}[htpb]
  \caption{Prompt components across different frameworks and documentations.}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l l l l l l}
    \toprule
    \textbf{LangGPT \cite{Wang2024LangGPTRS}} & \textbf{Elavis Saravia \cite{saravia2022prompt}} & \textbf{CRISPE \cite{ChatGPT3FreePromptList}} & \textbf{Google Cloud\cite{GoogleCloud}}   & \textbf{Merged} & \textbf{Definition}\\
    \midrule
    Profile & - & Capacity and Role & Persona  & \textbf{Profile/Role} & Who or what the model is acting as.\\
    \midrule
    \multirow{3}{*}{Goal} & \multirow{3}{*}{Instruction} & \multirow{3}{*}{Statement} & Objective & \multirow{3}{*}{\textbf{Directive}} & \multirow{3}{*}{\parbox{11.2cm}{The core intent of the prompt, often in the form of an instruction or question.}}\\
    & & & Instructions &\\
    & & & System Instructions  &\\
    \midrule
    Workflow & - & - & Reasoning Steps  & \textbf{Workflow} & Steps and processes the model should follow to complete the task.\\
    \midrule
   Initialization& \multirow{2}{*}{Context} & \multirow{2}{*}{Insights} & \multirow{2}{*}{Context}  & \multirow{2}{*}{\textbf{Context}} & \multirow{2}{*}{\parbox{11.2cm}{Background information and context that the model needs to refer to.}}\\
   Background  & &  &     \\
    \midrule
    Example & Input Data & - & Few-shot Examples   & \textbf{Examples} & Examples of what the response should look like.\\
    \midrule
    Output-format & \multirow{2}{*}{Output Indicator} & \multirow{2}{*}{Personality} & Response Format  & \multirow{2}{*}{\textbf{Output Format/Style}} & \multirow{2}{*}{The type, format, or style of the output.}\\
    Style &  &  & Tone  & \\
    \midrule
    \multirow{2}{*}{Constraints}& \multirow{2}{*}{-} & \multirow{2}{*}{-} & Constraints  &  \multirow{2}{*}{\textbf{Constraints}} & \multirow{2}{*}{\parbox{11.2cm}{Restrictions on what the model must adhere to when generating a response.}}\\
     & & & Safeguards & \\
    \midrule
    Skill & \multirow{2}{*}{-} & \multirow{2}{*}{Experiment} & \multirow{2}{*}{Recap}  &  \multirow{2}{*}{\textbf{Others}} & \multirow{2}{*}{-}\\
    Suggestion &  &  &  &  \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:merge}
\end{table}
\end{comment}

\input{tables/prompt_components}

We use the \llamaversion\ model to detect which components from the merged list are included in the prompts. For component detection, we design a prompt template that defines all available prompt components and specifies the expected JSON output format for the detection results. During analysis, we observe that the keys in the model's response often have slight variations from the predefined component names, such as using "Output" instead of "Output Format/Style". To address this issue, we apply similarity matching algorithms using the SequenceMatcher library to align the returned keys with the expected component names.

To evaluate the accuracy of component identification, we conduct both component-level and prompt-level human evaluations on a randomly selected 5\% sample of prompts. For component-level evaluation, precision is calculated as the proportion of components identified by the model that are correctly classified, compared to the human-labeled components:

\begin{equation}
\textit{precision} = \frac{\# \textit{correctly classified components}}{\# \textit{identified components}}
\end{equation}


For prompt-level evaluation, a prompt is classified as an exact match only if all identified components within the prompt are correct. If at least one component matched correctly but not all, the prompt is categorized as a partial match. To assess overall performance at the prompt level, we calculate both full match precision (P\textsubscript{full}) and partial match precision (P\textsubscript{partial}):

%\begin{equation}
%\textit{full match precision} = \frac{\textit{\#exact matched prompts}}{\textit{\#prompts with identified components}}
%\end{equation}
%\begin{equation}
%\textit{partial match precision} = \frac{\textit{\#exact/ partial matched prompts} }{\textit{\#prompts with identified components}}
%\end{equation}

\begin{equation}
P_{full} = \frac{\textit{\#exact matched prompts}}{\textit{\#prompts with identified components}}
\end{equation}

\begin{equation}
%P_{partial} = \frac{\textit{\#exact matched prompts} + \textit{\#partial matched prompts}}{\textit{\#prompts with identified components}}
P_{partial} = \frac{\textit{\#exact/ partial matched prompts} }{\textit{\#prompts with identified components}}
\end{equation}




The human evaluation results indicate that component-level precision is high, with an average precision of 86\% across all predefined component types. At the prompt level, the full match precision is 66\%, while the partial match precision is significantly higher at 99\%. Overall, the method demonstrates relatively high precision in component detection.

\noindent \textbf{Placeholder Analysis. } In this stage, we categorize placeholders within prompt templates through a two-step iterative process. First, we randomly select 100 prompt templates and manually classify each placeholder into predefined or newly identified categories as necessary. Next, we employ \gptversion\ to classify all prompt templates according to these preliminary categories and definitions. Following this, we conduct a human evaluation to verify the LLM's classifications, merging categories with low data representation and refining definitions where required. After adjusting the categories based on initial results, we perform a second round of LLM classification, followed by another human evaluation. This approach yields an overall classification accuracy of 81\% on a sample of 80 randomly selected records, ultimately identifying four primary placeholder categories as presented in Table~\ref{tab:placeholder}.

\input{tables/placeholder_type}

\noindent \textbf{Statistical Analysis and Pattern Analysis. } Using the theme classification, component analysis, and placeholder analysis results, we conduct a statistical analysis to examine the distribution of each category, as well as the frequency and relative positioning of elements at the word and phrase levels. From these statistical findings, we extract notable patterns that reveal structural and content trends within the prompt templates.

\subsection{Prompt Template Testing}
In this phase, we aim to assess the impact of various patterns identified in the previous analysis stage on the format-following and content-following of LLM outputs. 
For each identified pattern, we randomly sample prompt templates containing that pattern and use either the \gptversion\ model or real-world data sources to populate these templates. We then employ the \llamaversion\ and \gptversion\ models to generate outputs. Finally, we conduct a human evaluation to assess the quality of the generated outputs across different patterns, focusing on how well each pattern supports desired output characteristics.

% \begin{figure}[!h]
%     \centering    \includegraphics[width=1\textwidth]{figures/element_identification_workflow.png
%     }
%         \caption[Architecture of element identification]{Architecture of element identification.}
%     \label{fig:architecture_identification}
% \end{figure}

\begin{comment}
\begin{figure}[htpb]
    \centering
    \fbox{
    \parbox{0.95\textwidth}{
     \textbf{\# Instruction:}
        \newline
        Please carefully analyze the provided prompt and assign each identifiable complete sentence to one of the elements listed below. Avoid using phrases or single words unless they form a complete idea. Ensure that each part is distinctly categorized to prevent overlap.
        \newline
        \newline
        \textbf{\#\# Prompt:}
        \newline
        '''\{prompt\}'''
        \newline
        \newline
        \textbf{\#\# Element Definitions:}
        \newline
        1. Profile/Role: Who or what the model is acting as.
        \newline
        2. Directive: The core intent of the prompt, often in the form of an instruction or question.
        \newline
        3. Workflows: Steps and processes the model should follow to complete the task.
        \newline
        4. Context: Background information and context that the model needs to refer to.
        \newline
        5. Examples: Examples of what the response should look like.
        \newline
        6. Output Format/Style: The type, format, or style of the output.
        \newline
        7. Constraints: Restrictions on what the model must adhere to when generating a response.
        \newline
        8. Others: Any other elements that do not fit into the above categories.
        \newline
        \newline
        \textbf{\#\# Output Format:}
        \newline
        Please return the output in the following JSON structure without additional commentary or explanation, and ensure to assign unique content to each category to avoid any overlaps:
        \newline
        '''
        
        \{
        
        "profile/role": "",
        
        "directive": "",
        
        "workflows": "",
        
        "context": "",
        
        "examples": "",
        
        "output format/style": "",
        
        "constraints": "",
        
        "others": ""
        \}
        
        '''
    }
    }
    \caption{Prompts used for element detection. \chen{Not necessary, make it one table/list in main text is enough}}
    \label{fig:prompt_element_detection}
\end{figure}
\end{comment}

==> sections/Related_Work.tex <==
\section{Related Work}

% \junjie{\noindent \textbf{LLM4SE.?} Recent studies have shown the potential of LLM to enhance software engineering tasks. Fan \etal~\cite{Fan2023LargeLM} conducted a comprehensive survey in this area, focusing on challenges and future trends. Zhang \etal~\cite{Zhang2023ASO} summarized various model architectures, pre-training objectives, and downstream tasks of software engineering.} 

% \junjie{Lanciano \etal~\cite{Lanciano2023AnalyzingDD} explored using LLMs with few-shot learning prompts to analyze declarative deployment code and provide quality assurance recommendations to developers. .... Different from these studies, our work specifically focuses on the practical application of prompt engineering in real development environments.}

\noindent \textbf{Software Engineering for LLM.} Software Engineering for Large Language Models (SE4LLM) is an emerging field focused on applying software engineering principles to the development and deployment of LLMs. Recent research addresses key areas such as efficiency, security, and interpretability. For instance, Aminabadi~\etal~\cite{aminabadi2022deepspeed} implemented the DeepSpeed Inference system to optimize the system stack for efficient transformer model inference, particularly across varying model sizes and GPU resources. Touvron~\etal~\cite{Touvron2023Llama2O} emphasized security as a critical consideration in Llama 2 for LLM deployment, which incorporates safety-focused data annotation and red-team testing to enhance model robustness. Goyal~\etal~\cite{goyal2024llmguard} proposed LLMGuard to offer a modular monitoring approach by employing a suite of detectors targeting issues like personal information leakage, racial bias, and toxic content, ensuring safer, enterprise-grade LLM usage. Dunefsky~\etal~\cite{dunefsky2024transcoders} proposed transcoders improve interpretability within LLMs by translating densely activating sublayers into interpretable, sparse subcomponents, effectively enabling more accessible circuit analysis for understanding model behaviors.
%In contrast to these works, which focus on runtime optimizations and analysis of LLM internal mechanisms, our research addresses the interaction stage between users and LLM applications by analyzing prompt templates. 
In contrast to these works, which address post-deployment challenges such as runtime optimizations and analysis of LLM internal mechanisms, our research focuses on the pre-deployment phases. In particular, we address the interaction stage between users and LLM applications by analyzing prompt templates. 
This approach provides actionable insights and optimizations before the model executes a prompt, guiding developers in creating more effective templates to enhance user-LLM interactions. Our work complements existing methods by offering pre-execution guidance, adding a layer of prompt analysis that can support runtime-focused studies in optimizing LLM-based applications.

%\junjie{\url{https://arxiv.org/pdf/2403.00826} could this one also be added in this part? "a tool that monitors user interactions with an LLM application and flags content against specific behaviours or conversation topics and employs an ensemble of detectors"}

\noindent \textbf{Prompt Engineering. } Prompt engineering has become essential for guiding LLMs, but the variability in natural language presents challenges for achieving clarity and consistency. Recent research explores common prompt elements and effective structural patterns. For example, Wang \etal~\cite{Wang2024LangGPTRS} introduced a reusable framework based on programming constructs to standardize prompt elements. Reynolds and McDonell \cite{reynolds2021prompt} emphasized task-specific instructions and formatting to enhance model performance. Additionally, Liu \etal~\cite{liu2023instruction} and Cuconasu \etal~\cite{cuconasu2024power} examined how positional sequencing of elements impacts quality in generation and RAG tasks. Finally, Sclar \etal~\cite{sclar2023quantifying} found that minor prompt changes, like punctuation or formatting, can significantly affect model responses, underscoring the importance of refined prompt design. Unlike prior research, which explores the design of prompts in general usage, our study specializes in systematically analyzing prompt templates in LLM-powered applications. Drawing on the idea of prior studies, we determine and examine the common components and structural patterns within prompt templates, including positional arrangements. Notably, we conduct a detailed analysis of placeholders, which are a unique feature of prompt templates that makes them more reusable than prompts. To the best of our knowledge, our research is the first to explore prompt templates in FMware applications, offering developers insights into crafting effective templates to address diverse user inputs.

% \junjie{\noindent \textbf{Prompt engineering template.}} Prompt engineering has emerged as a novel paradigm for instructing large language models (LLMs) to implement user requirements. Since prompts are typically written in natural language, the inherent ambiguity and variability of natural language pose challenges in crafting clear and effective prompts. As a result, recent research has focused on analyzing how prompts are written and developing guidelines to improve prompt clarity and effectiveness.

% Previous research identifies commonalities among real-world user prompts as specific prompt elements. By analyzing how users construct various types of prompt elements, researchers can extract universal writing guidelines. Wang \etal~\cite{Wang2024LangGPTRS} analyzed prompt design by introducing a structured and reusable framework modeled after programming languages, breaking down prompts into distinct elements. Reynolds and McDonell \cite{reynolds2021prompt} explored how to design effective prompts by focusing on key elements like task-specific instructions, and format specifications to improve LLM performance across tasks. They analyzed how various prompt structures, including instructional clarity and contextual information, influence the quality of the generated outputs, and the results showed that well-structured prompts can enable zero-shot performance to surpass few-shot methods, reducing the need for multiple examples and improving task effectiveness.

% In addition to the structural composition of prompts, the positional arrangement of prompt elements has also been studied. Liu \etal~\cite{liu2023instruction} investigated how the position of instructions in sequence generation tasks affects the output quality. Cuconasu \etal~\cite{cuconasu2024power} studied how the position of the gold document among the retrieved documents and its distance from the user query affect the performance of Retrieval-Augmented Generation (RAG) systems. Mao \etal~\cite{mao2023prompt} examined the prompt positions used in previous studies and adjusted them to investigate their impact on model performance.

% Recent research on prompt design also investigates how small modifications in prompt structure, phrasing, or formatting impact model outputs. For example, Sclar \etal~\cite{sclar2023quantifying} analyzed the effects of seemingly minor changes in prompt formatting, such as adjusting word order, punctuation, or adding unnecessary words, on large language model performance. Similarly, Salinas and Morstatter \etal~\cite{salinas2024butterfly} used text classification tasks to examine the impact of small prompt variations, including changes in output format, added spaces, punctuation modifications, and jailbreak techniques, on the decisions of large language models.



==> sections/Threat_to_Validity.tex <==
\section{Threat to Validity}
We have identified the following limitations to our research:

First, our investigation focuses on frequently used themes, components, and patterns in prompt templates with a significant impact on LLM output quality. However, this approach may overlook other factors that could also affect output quality. To mitigate this limitation, we merged the elements defined from different sources to obtain a broader range of influential factors. In future work, we will expand our research scope to identify additional elements and patterns influencing LLM outputs, aiming for a more exhaustive understanding of prompt engineering.

Additionally, our experiments were primarily conducted using the \llamaversion\ and \gptversion\ models. \llamaversion\ model is widely used in LLM-powered applications due to its open-source, cost-effectiveness, and data protection characteristics. Future research should investigate how prompt variations affect a range of models, architectures, and training datasets. Investigating these aspects across diverse models would provide a more comprehensive view of prompt engineering’s effects on model behavior and performance, offering broader implications for LLM-powered application development.

==> sections/Threat_to_Validity_2column.tex <==
\section{Threat to Validity}
We have identified the following limitations to our research:

First, our investigation focuses on frequently used themes, components, and patterns in prompt templates with a significant impact on LLM output quality. However, this approach may overlook other factors that could also affect output quality. To mitigate this limitation, we merged the elements defined from different sources to obtain a broader range of influential factors. In future work, we will expand our research scope to identify additional elements and patterns influencing LLM outputs, aiming for a more exhaustive understanding of prompt engineering.

Additionally, our experiments were primarily conducted using the \llamaversion\ and \gptversion\ models, which are widely used in \llmapps. Future research should investigate how prompt variations affect a range of models, architectures, and training datasets. Investigating these aspects across diverse models would provide a more comprehensive view of prompt engineering’s effects on model behavior and performance, offering broader implications for \llmapp development.

==> tables/constraint.tex <==
\begin{table}[htpb]
\caption{\rmfamily Output quality under three json output format pattern. \chen{Too easy, no need to write it into one table.}}
\rmfamily
\centering
%\resizebox{\textwidth}{!}{
\label{tab:constarint}
%\setlength\tabcolsep{20pt}
\begin{tabular}{ll}
\toprule
                       & \textbf{Output Simplicity} \\ 
                       \midrule
Prompt                 & 0.4               \\ 
\midrule
Prompt with Constraint & 0.8               \\ 
\bottomrule
\end{tabular}
%}
\end{table}

==> tables/placeholder_type.tex <==
\begin{table}[htpb]
\centering
\caption{Placeholder Type. \chen{Should also be put into RQ3 and merged with Figure 10.}}
\resizebox{\linewidth}{!}{
    \label{tab:placeholder}
    \begin{tabular}{l p{0.5\linewidth} p{0.3\linewidth}}
        \toprule
        \textbf{Category} & \textbf{Description}  & \textbf{Example}\\
        \midrule
        User Question & Queries or questions provided by users. & \{\{question\}\}, \{\{query\}\}\\
        Contextual Information & Background or supplementary input that helps set the stage for the task but is not the primary focus. & \{\{chat\_history\}\}, \{\{background\_info\}\} \\
        Knowledge Input  & The core content that the prompt directly processes or manipulates. & \{\{document\}\}\\
        Metadata/Short Phrases & Brief inputs or settings that define specific parameters or goals for the task. & \{\{language\}\}, \quad \{\{username\}\} \\
        \bottomrule
    \end{tabular}
}
\end{table}

==> tables/placeholder_type_2.tex <==
\begin{table}[htpb]
\centering
\caption{Relative frequency distribution of placeholder type categorized by LLM.}
\resizebox{\linewidth}{!}{
    \label{tab:placeholder_2}
    \begin{tabular}{l p{0.5\linewidth} p{0.3\linewidth} l}
        \toprule
        \textbf{Category} & \textbf{Description}  & \textbf{Example} & \textbf{Frequency}\\
        \midrule
        User Question & Queries or questions provided by users. & \{\{question\}\}, \{\{query\}\} & 14.0\%\\
        \rowcolor{gray!10} Contextual Information & Background or supplementary input that helps set the stage for the task but is not the primary focus. & \{\{chat\_history\}\}, \{\{background\_info\}\} & 12.8\%\\
        Knowledge Input  & The core content that the prompt directly processes or manipulates. & \{\{document\}\}& 34.7\%\\
        \rowcolor{gray!10} Metadata/Short Phrases & Brief inputs or settings that define specific parameters or goals for the task. & \{\{language\}\}, \quad \{\{username\}\} & 38.4\% \\
        \bottomrule
    \end{tabular}
}
\end{table}

==> tables/placeholer_content_length.tex <==
\begin{table}[htpb]
\caption{\rmfamily Output quality under different knowledge input position and placeholder content length. \chen{For long placeholder content, why is the performance of content following even better than short ones? } }
\rmfamily
\centering
\resizebox{\linewidth}{!}{
\label{tab:placeholer_length}
%\setlength\tabcolsep{10pt}
\begin{tabular}{p{2cm}lcccc}
\toprule
\multirow{3}{=}{\textbf{Length of Placeholder Content}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{ Content Following }} & \multicolumn{2}{c}{\textbf{ Content Following }} \\ 
&  &  \multicolumn{2}{c}{\textbf{(Question)}} & \multicolumn{2}{c}{\textbf{(Task Intent)}}\\
                              &                          & Pattern 1       & Pattern 2        & Pattern 1             & Pattern 2             \\ 
\midrule
\multirow{2}{*}{Short}        & LLaMA                    & 4.61                & \textbf{4.95}                & 4.44                   & 4.44                  \\
                              & GPT                      & 4.62                & \textbf{4.89}                & 4.56                   & \textbf{4.89}                  \\ 
\midrule
\multirow{2}{*}{Medium}       & LLaMA                    & 4.39                & \textbf{4.67}                & 3.56                   & \textbf{4.56}                  \\
                              & GPT                      & \textbf{4.78}                & 4.44                & 4.56                   & 4.56                  \\ 
\midrule
\multirow{2}{*}{Long}         & LLaMA                    & 4.56                & \textbf{4.89}                & 3.17                   & \textbf{4.89}                  \\
                              & GPT                      & 4.44                & \textbf{4.78}                & 3.67                   & \textbf{4.34}                  \\ 
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\footnotesize
\item Pattern 1 is Task Intent -> \{Knowledge Input\} -> \{User Question\}. Pattern 2 is \{Knowledge Input\} -> Task Intent -> \{User Question\}.
\end{tablenotes}
\end{table}

==> tables/predifined_theme.tex <==
\begin{table}[htpb]
    \centering
\caption{Predefined Task theme categories. \chen{1. reasoning and planning sound more like capabilities, rather than ``task'' as they are needed in all tasks. 2. I suggest to put it into next section, the result analysis part, rather than here. Please merge it with Figure 4. That will also help save some space. 3. Please use gray and white to separate table rows to enhance its readability, as there are many rows.}\mao{Need to add a column of frequency(percentage) at the end}}
\resizebox{\linewidth}{!}{
    \label{tab:task_tags}
    \begin{tabular}{ll}
        \toprule
        \textbf{Task Tag} & \textbf{Description} \\
        \midrule
            Information seeking & Users ask for specific information or facts about various topics. \\
         \rowcolor{gray!10} Reasoning & Queries require logical thinking, problem-solving, or complex idea processing. \\
        Planning & Users need assistance in creating plans or strategies for activities/projects. \\
        \rowcolor{gray!10} Editing & Involves editing, rephrasing, proofreading, or general writing composition tasks. \\
        Coding \& Debugging & Users seek help with writing, reviewing, or fixing programming code. \\
        \rowcolor{gray!10} Math & Queries related to mathematical concepts, problems, and calculations. \\
        Role playing & Users engage in scenarios requiring ChatGPT to adopt a character or persona. \\
        \rowcolor{gray!10} Data analysis & Requests involve interpreting data, statistics, or performing analytical tasks. \\
        Creative writing & Users seek assistance with crafting stories, poems, or other creative texts. \\
        \rowcolor{gray!10} Advice seeking & Users ask for recommendations or guidance on personal or professional issues. \\
        Brainstorming & Involves generating ideas, creative thinking, or exploring possibilities. \\
         \rowcolor{gray!10}Others & Queries that do not fit into the above categories or are of a miscellaneous nature. \\
        \bottomrule
    \end{tabular}
}
\end{table}

==> tables/predifined_theme_2.tex <==
\begin{table}[htpb]
    \centering
\caption{Predefined Task theme categories. \chen{1. reasoning and planning sound more like capabilities, rather than ``task'' as they are needed in all tasks. 2. I suggest to put it into next section, the result analysis part, rather than here. Please merge it with Figure 4. That will also help save some space. 3. Please use gray and white to separate table rows to enhance its readability, as there are many rows.}\mao{Need to add a column of frequency(percentage) at the end} \junjie{should it be sorted by frequency, and put "others" at the end?}\mao{better to be sorted, and put "others" at the end}}
\resizebox{\linewidth}{!}{
    \label{tab:task_tags}
    \begin{tabular}{lll}
        \toprule
        \textbf{Task Tag} & \textbf{Description}&\textbf{Frequency} \\
        \midrule
            Information seeking & Users ask for specific information or facts about various topics.  &  42.2\% \\
        \rowcolor{gray!10} Editing & Involves editing, rephrasing, proofreading, or general writing composition tasks. & 11.6\% \\
        Coding \& Debugging & Users seek help with writing, reviewing, or fixing programming code.  & 10.3\%\\
    \rowcolor{gray!10} Creative writing & Users seek assistance with crafting stories, poems, or other creative texts.& 6.8\% \\
Reasoning & Queries require logical thinking, problem-solving, or complex idea processing.& 6.6\% \\
\rowcolor{gray!10} Data analysis & Requests involve interpreting data, statistics, or performing analytical tasks. & 5.4\%\\
Role playing & Users engage in scenarios requiring ChatGPT to adopt a character or persona. & 3.2\%\\
\rowcolor{gray!10} Planning & Users need assistance in creating plans or strategies for activities/projects. & 2.9\%\\
    Advice seeking & Users ask for recommendations or guidance on personal or professional issues. & 1.7\% \\
   \rowcolor{gray!10}    Brainstorming & Involves generating ideas, creative thinking, or exploring possibilities. & 1.6\%\\

 Math & Queries related to mathematical concepts, problems, and calculations.  & 0.8\% \\


         \rowcolor{gray!10}Others & Queries that do not fit into the above categories or are of a miscellaneous nature.& 6.8\% \\
        \bottomrule
    \end{tabular}
}
\end{table}
